Model-Powered Conditional Independence Test

We consider the problem of non-parametric Conditional Independence testing (CI testing) for continuous random variables. Given i.i.d samples from the joint distribution $f(x,y,z)$ of continuous random vectors $X,Y$ and $Z,$ we determine whether $X \perp Y | Z$. We approach this by converting the conditional independence test into a classification problem. This allows us to harness very powerful classifiers like gradient-boosted trees and deep neural networks. These models can handle complex probability distributions and allow us to perform significantly better compared to the prior state of the art, for high-dimensional CI testing. The main technical challenge in the classification problem is the need for samples from the conditional product distribution $f^{CI}(x,y,z) = f(x|z)f(y|z)f(z)$ -- the joint distribution if and only if $X \perp Y | Z.$ -- when given access only to i.i.d. samples from the true joint distribution $f(x,y,z)$. To tackle this problem we propose a novel nearest neighbor bootstrap procedure and theoretically show that our generated samples are indeed close to $f^{CI}$ in terms of total variational distance. We then develop theoretical results regarding the generalization bounds for classification for our problem, which translate into error bounds for CI testing. We provide a novel analysis of Rademacher type classification bounds in the presence of non-i.i.d near-independent samples. We empirically validate the performance of our algorithm on simulated and real datasets and show performance gains over previous methods.

==> Introduction.tex <==
%Rough Story....
%
%(i) Three areas where CI tests are the main work-horse:
%
%(1) Markov Blanket Estimation with cites.
%
%(2) Bayesian Network Learning - add cites
%
%(3) Causal Structure learning - discuss both constraint based and score based contributions. 
%
%Prior work on parametric and non-parametric CI. Kernel based methods. Discuss run time and dimensionality hit. 
%
%(ii) Discuss that ours is a modular approach- simple bootstrap followed by powerful classifiers. Classifiers can be flexibly chosen with domain knowledge, and any advancement in this field implies an advancement in ours. Discuss dimension issues. 
%
%(iii) List main contributions:
%
%(1) Reduction to classification with NNB.
%
%(2) Guarantees for NNB
%
%(3) Novel guarantees for non-i.i.d classification
%
%(4) Empirical Performance. 

%%%%%%%%%%%%%%%%%%%%%%%%%Start Intro%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
Conditional Independence is a fundamental concept with a wide range of applications in statistics and machine learning~\cite{dawid1979conditional}. Given three sets of random variables $X$, $Y$ and $Z$, $X$ is conditionally independent of $Y$ given $Z$ ($X \independent Y \vert Z$), when the joint distribution $f_{X,Y,Z}(x,y,z)$ factorizes as $f_{X,Y,Z}(x,y,z) = f_{X|Z}(x|z)f_{Y|Z}(y|z)f_{Z}(z)$. The problem of \textit{Conditional Independence Testing} (CI Testing) can be defined as: Given $n$ i.i.d samples from $f_{X,Y,Z}(x,y,z)$, distinguish between the two hypothesis $\mathcal{H}_0:$ $X \independent Y \vert Z$ and $\mathcal{H}_1:$ $X \centernot{\independent} Y \vert Z$. CI tests are fundamental tools for learning Bayesian networks~\cite{koller2009probabilistic}, causal inference~\cite{pearl2009causality} and feature selection through Markov Blankets~\cite{koller1996toward}. 

In causal structure learning, results of CI tests among the nodes of a causal graph~\cite{pearl2009causality} are vital inputs to popular constraint based algorithms~\cite{kalisch2007estimating,tsamardinos2006max}. A key property is that given two variables on a causal graph $X$ and $Y$ and a set of other variables $\mathcal{S}$ (also nodes in the causal graph), $X \independent Y \vert \mathcal{S}$, implies the absence of an edge between $X$ and $Y$. Some of the more recent score-based methods of causal inference also rely on effective CI tests~\cite{brenner2013sparsityboost}. Similarly in the field of learning Bayesian networks, results from CI tests are used to discover edges between random variables that form the nodes of the network~\cite{spirtes2000causation,cheng1998learning,de2000new}. CI tests are also useful in the field of feature selection for high-dimensional supervised learning problems~\cite{koller1996toward, xing2001feature}. In a classification problem we are given a large set of features $\mathcal{F}$ and class-labels $C$ i.e each data-point has $\vert \mathcal{F}\vert$ features and a class-label. The key observation~\cite{koller1996toward} is that: Given a feature $F_i$ and a set of features $M_i \in \mathcal{F}$ (s.t. $F_i \notin M_i$), if $F_i \independent \mathcal{F}\setminus \{M_i \cup F_i\}, C \vert M_i$, then the feature $F_i$ can be safely removed without hurting the accuracy of learning. This property can be used to prune the set of features for a high-dimensional problem.

The problem of CI testing is much harder than testing for independence (i.e whether $X \independent Y$)~\cite{bergsma2004testing}, especially when the random variables $X,Y$ and $Z$ are continuous valued. When $Z$ is discrete, CI tests can be reduced to independence tests by partitioning the data-set according to values of $Z$, and testing for independence separately in each partition. In the continuous case, traditional methods focus on parametric assumptions like linear relations between the random variables with additive Gaussian noise, where the problem reduces to testing for correlations~\cite{lawrance1976conditional}. Our focus is on \textit{non-parametric} CI testing for continuous random variables, i.e. determining CI relations without such simplifying assumptions. 

Some of the earlier methods for non-parametric CI testing, either involve discretizing $Z$ into sets of bins~\cite{margaritis2005distribution}, or involve estimating the marginal densities $f_{X \vert Z}(.)$ and $f_{Y \vert Z}(.)$~\cite{su2007consistent}. Unfortunately, these methods suffer from the curse of dimensionality, when the dimension of $Z$ is greater than $1$. Recently, powerful kernel based methods for non-parametric CI testing have been proposed that are accurate even for moderate values of the dimensions of $Z$~\cite{gao2016demystifying,strobl2017approximate,zhang2012kernel,doran2014permutation}. Many of these approaches are based on the observation in~\cite{fukumizu2004dimensionality}, that non-parametric CI relations can be characterized using covariance operators in
the reproducing kernel Hilbert spaces (RKHS). However, even these kernel based methods have issues in accuracy of the test when the dimension of the conditioning set is more than $70$~\cite{doran2014permutation} and also incur prohibitive running times when the number of i.i.d samples $n$ supplied, is large~\cite{strobl2017approximate}. RCIT~\cite{strobl2017approximate} is in fact a randomized version of KCIT~\cite{zhang2012kernel} that attempts to reduce the run-time when the number of samples is large. 

\begin{figure}[h]
	\centering
	\includegraphics[width=9cm,height=6cm]{illustrate.pdf}
	\caption{Illustration of our methodology. A part of the original samples are kept aside in $\mathcal{U}$. The rest of the samples are used in our nearest neighbor boot-strap to generate a data-set $\mathcal{U}'$ which is close to $f^{CI}$ in distribution. The samples are labeled as shown and a classifier is trained on a training set. The test error is measured on a test set there-after. If the test-error is close to $0.5$, then $\mathcal{H}_0$ is not rejected, however if the test error is low then $\mathcal{H}_0$ is rejected.}
	\label{fig:illustrate}
\end{figure}

In this paper, we take a modular approach (illustrated in Fig.~\ref{fig:illustrate}), which reduces the problem of CI testing to Binary Classification~\cite{boucheron2005theory} as follows:

$(i)$ The first module in our method is a Nearest-neighbor based boot-strap which simulates $n/2$ new samples, when supplied with $n$ i.i.d samples from the joint distribution $f_{X,Y,Z}(x,y,z)$. In Sections~\ref{sec:Algorithm} and \ref{sec:results}, we show that these new samples are in fact close in variational distance (defined in Section~\ref{sec:results}) to the distribution $f^{CI}(x,y,z) = f_{X|Z}(x|z)f_{Y|Z}(y|z)f_Z(z)$. As shown in Fig.~\ref{fig:illustrate}, $n/3$ original samples are kept aside in $\mathcal{U}$, while the remaining $2n/3$ are used to generate $n/3$ samples (close to $f^{CI}$ in distribution) in $\mathcal{U}'$, using our nearest-neighbor bootstrap. 

$(ii)$ Subsequently, the original samples in $\mathcal{U}$ are labeled $1$ while the new samples simulated from the nearest-neighbor bootstrap are labeled $0$. This labeled data-set is then broken into training and test sets. 

$(iii)$ Given the labeled training data-set (from step (ii)), we train powerful classifiers such as gradient boosted trees~\cite{chen2016xgboost} or deep neural networks~\cite{krizhevsky2012imagenet} which attempt to learn the classes of the samples. If the trained classifier has good accuracy over the test set, then intuitively it means that the joint distribution $f_{X,Y,Z}(.)$ is distinguishable from $f^{CI}$ (note that the generated samples labeled 0 are close in distribution to $f^{CI}$). Therefore, we reject $\mathcal{H}_0$. On the other hand, if the classifier has accuracy close to random guessing, then $f_{X,Y,Z}(.)$ is in fact close to $f^{CI}$, and we fail to reject $\mathcal{H}_0$. 

The advantage of this modular approach is that we can harness the power of supervised learning tools (in step (iii) above), which have good accuracies in high-dimensions. Further, any improvements in the field of binary classification imply an advancement in our CI test. Moreover, there is added flexibility in choosing the best classifiers based on domain knowledge about the data-generation process. Binary classification has been used before for two-sample testing in~\cite{lopez2016revisiting}. Finally, the nearest-neighbor based bootstrap is efficient as well, owing to fast algorithms for identifying nearest-neighbors~\cite{ramasubramanian1992fast}. In the following section, we list our main contributions. 

\subsection{Main Contributions}
\label{contri}
The main contributions of this paper are as follows:

$(i)$ {\bf (Nearest-Neighbor Bootstrap)} We propose a nearest-neighbor based bootstrap method to produce samples whose distributions are close to $f^{CI}$, given access to $n$ i.i.d samples from the joint $f_{X,Y,Z}(x,y,z)$. This is Algorithm~\ref{alg:NNB} in our paper. We prove that the variational distance between the distribution of any one of the samples returned by Algorithm~\ref{alg:NNB} and $f^{CI}$ (conditionally independent distribution) is $O((1/n)^{1/2d_z})$ under mild smoothness assumptions on $f_{X,Y,Z}(x,y,z)$. 

$(ii)$ {\bf (Reduction to Classification)} We reduce the problem of CI tests into a binary classification problem, through our nearest neighbor bootstrap. As shown in Fig.~\ref{fig:illustrate}, we withhold $n/3$ of the original samples in data-set $\mathcal{U}$, while $2n/3$ of the original samples are passed through the nearest neighbor boot-strap to create $n/3$ samples (in $\mathcal{U}'$), that are close to $f^{CI}$ in distribution.  The samples in $\mathcal{U}$ are labeled $1$ and the ones in $\mathcal{U}'$ are labeled $0$. This labeled data-set is broken into training set $\mathcal{D}_r$ and test set $\mathcal{D}_e$. A classifier $\hat{g}$ is trained on $\mathcal{D}_r$. 

The key idea is that if the original samples are in fact CI ($\mathcal{H}_0$ holds), then the two data-sets cannot be distinguished and the test error $\hat{L}(\hat{g},\mathcal{D}_{e})$ will be close to $0.5$ (random guessing). However, if $\mathcal{H}_1$ holds, then the classifier will be able to differentiate between the data-sets i.e. $\hat{L}(\hat{g},\mathcal{D}_{e}) < 0.5$ would be observed. We provide a detailed pseudo-code in Algorithm~\ref{alg:ccitv1}.

$(iii)$ {\bf (Bias Corrected Algorithm)} We provide an improved algorithm in Algorithm~\ref{alg:ccitv2}. The samples generated in the nearest-neighbor boot-strap are close to $f^{CI}$ but the variational distance is not exactly equal to $0$ for finite $n$. Moreover the bootstrapped samples are not exactly i.i.d. Therefore, the trained classifier is expected to have a bias i.e the classifier can achieve a test loss slightly less than 0.5, even when $\mathcal{H}_0$ holds. In Algorithm~\ref{alg:ccitv2}, we propose a simple idea to rectify this bias.  

%(i) a part of the original i.i.d samples are labeled $1$ (ii) the other part of the original samples are supplied to Algorithm~\ref{alg:NNB} to produce samples that are close to $f^{CI}$. These new samples are labeled $0$. (iii) A subset labeled samples are supplied to a binary classifier for training. The trained classifier is tested on a validation set (separate from the training set). If the trained classifier has good accuracy over a validation set, then intuitively it means that the joint distribution $f_{X,Y,Z}(.)$ is distinguishable from $f^{CI}$ (note that the generated samples labeled 0 are close in distribution to $f^{CI}$). Therefore, we reject $\mathcal{H}_0$. On the other hand, if the classifier has accuracy close to random guessing, then $f_{X,Y,Z}(.)$ is in fact close to $f^{CI}$, and we fail to reject $\mathcal{H}_0$.

$(iv)$ {\bf (Novel Generalization Guarantees for Classification)} The samples generated by the nearest-neighbor bootstrap are not i.i.d any more, but they are \textit{close} to i.i.d. We show that even though these samples are not i.i.d, generalization bounds (similar to~\cite{boucheron2005theory} ) for the risk of classifiers trained on them, still hold. (add details about the result). In proving this, we provide a novel analysis for Rademacher type bounds (refer to ~\cite{boucheron2005theory}) for non-i.i.d samples, which relate the classification accuracy to the number of samples and the $VC$-dimension~\cite{vapnik2015uniform} of the class of functions in the classifier. This analysis technique may be of independent interest. 

$(v)$ {\bf (Empirical Validation)} We perform better on real and simulated data..........need more evidence to write. 



==> Introductionv2.tex <==
%Rough Story....
%
%(i) Three areas where CI tests are the main work-horse:
%
%(1) Markov Blanket Estimation with cites.
%
%(2) Bayesian Network Learning - add cites
%
%(3) Causal Structure learning - discuss both constraint based and score based contributions. 
%
%Prior work on parametric and non-parametric CI. Kernel based methods. Discuss run time and dimensionality hit. 
%
%(ii) Discuss that ours is a modular approach- simple bootstrap followed by powerful classifiers. Classifiers can be flexibly chosen with domain knowledge, and any advancement in this field implies an advancement in ours. Discuss dimension issues. 
%
%(iii) List main contributions:
%
%(1) Reduction to classification with NNB.
%
%(2) Guarantees for NNB
%
%(3) Novel guarantees for non-i.i.d classification
%
%(4) Empirical Performance. 

%%%%%%%%%%%%%%%%%%%%%%%%%Start Intro%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
Conditional Independence is a fundamental concept with a wide range of applications in statistics and machine learning~\cite{dawid1979conditional}. Given three sets of random variables $X$, $Y$ and $Z$, $X$ is conditionally independent of $Y$ given $Z$ ($X \independent Y \vert Z$), when the joint distribution $f_{X,Y,Z}(x,y,z)$ factorizes as $f_{X,Y,Z}(x,y,z) = f_{X|Z}(x|z)f_{Y|Z}(y|z)f_{Z}(z)$. The problem of \textit{Conditional Independence Testing} (CI Testing) can be defined as: Given $n$ i.i.d samples from $f_{X,Y,Z}(x,y,z)$, distinguish between the two hypothesis $\mathcal{H}_0:$ $X \independent Y \vert Z$ and $\mathcal{H}_1:$ $X \centernot{\independent} Y \vert Z$. CI tests are fundamental tools for learning Bayesian networks~\cite{koller2009probabilistic}, causal inference~\cite{pearl2009causality} and feature selection through Markov Blankets~\cite{koller1996toward}. 

In causal structure learning, results of CI tests among the nodes of a causal graph~\cite{pearl2009causality} are vital inputs to popular constraint based algorithms~\cite{kalisch2007estimating,tsamardinos2006max}. A key property is that given two variables on a causal graph $X$ and $Y$ and a set of other variables $\mathcal{S}$ (also nodes in the causal graph), $X \independent Y \vert \mathcal{S}$, implies the absence of an edge between $X$ and $Y$. Some of the more recent score-based methods of causal inference also rely on effective CI tests~\cite{brenner2013sparsityboost}. Similarly in the field of learning Bayesian networks, results from CI tests are used to discover edges between random variables that form the nodes of the network~\cite{spirtes2000causation,cheng1998learning,de2000new}. CI tests are also useful in the field of feature selection for high-dimensional supervised learning problems through Markov blankets~\cite{koller1996toward, xing2001feature}. 

CI testing is fundamentally much harder than testing for independence (i.e whether $X \independent Y$)~\cite{bergsma2004testing}. When $Z$ is discrete, CI tests can be reduced to independence tests by partitioning the data-set according to values of $Z$, and testing for independence separately in each partition. The continuous setting is more difficult, where traditional methods focus on parametric assumptions like linear relations between the random variables with additive Gaussian noise, where the problem reduces to testing for correlations~\cite{lawrance1976conditional}. Our focus is on \textit{non-parametric} CI testing for continuous random variables, i.e. determining CI relations without such simplifying assumptions. 

Some of the earlier methods for non-parametric CI testing, either involve discretizing $Z$ into sets of bins~\cite{margaritis2005distribution}, or involve estimating the marginal densities $f_{X \vert Z}(.)$ and $f_{Y \vert Z}(.)$~\cite{su2007consistent}. Unfortunately, these methods do not perform well in higher dimensions of $Z$. Recently, powerful kernel based methods for non-parametric CI testing have been proposed that are accurate even for moderate values of the dimensions of $Z$~\cite{gao2016demystifying,strobl2017approximate,zhang2012kernel,doran2014permutation}. 
%Many of these approaches are based on the observation in~\cite{fukumizu2004dimensionality}, that non-parametric CI relations can be characterized using covariance operators in the reproducing kernel Hilbert spaces (RKHS). 
However, even these kernel based methods have issues in accuracy of the test when the dimension of the conditioning set is large~\cite{doran2014permutation} and also incur prohibitive running times when the number of samples ($n$) is large~\cite{strobl2017approximate}. 

\begin{figure}[h]
	\centering
	\includegraphics[width=7cm,height=4.5cm]{illustrate.pdf}
	\caption{Illustration of our methodology. A part of the original samples are kept aside in $\mathcal{U}$. The rest of the samples are used in our nearest neighbor boot-strap to generate a data-set $\mathcal{U}'$ which is close to $f^{CI}$ in distribution. The samples are labeled as shown and a classifier is trained on a training set. The test error is measured on a test set there-after. If the test-error is close to $0.5$, then $\mathcal{H}_0$ is not rejected, however if the test error is low then $\mathcal{H}_0$ is rejected.}
	\label{fig:illustrate}
\end{figure}

In this paper, we take a modular approach (illustrated in Fig.~\ref{fig:illustrate}), which reduces the problem of CI testing to Binary Classification~\cite{boucheron2005theory} as follows:

\setword{$(i)$}{step1} The first module in our method is a Nearest-neighbor based boot-strap which simulates $n/2$ new samples, when supplied with $n$ i.i.d samples from the joint distribution $f_{X,Y,Z}(x,y,z)$. In Sections~\ref{sec:Algorithm} and \ref{sec:results}, we show that these new samples are in fact close in variational distance (defined in Section~\ref{sec:results}) to the distribution $f^{CI}(x,y,z) \triangleq f_{X|Z}(x|z)f_{Y|Z}(y|z)f_Z(z)$. As shown in Fig.~\ref{fig:illustrate}, $n/3$ original samples are kept aside in $\mathcal{U}$, while the remaining $2n/3$ are used to generate $n/3$ samples (close to $f^{CI}$ in distribution) in $\mathcal{U}'$, using our nearest-neighbor bootstrap. 

\setword{$(ii)$}{step2} Subsequently, the original samples in $\mathcal{U}$ are labeled $1$ while the new samples simulated from the nearest-neighbor bootstrap are labeled $0$. This data-set is then broken into training and test sets. 

\setword{$(iii)$}{step3} Given the labeled training data-set (from step (ii)), we train powerful classifiers such as gradient boosted trees~\cite{chen2016xgboost} or deep neural networks~\cite{krizhevsky2012imagenet} which attempt to learn the classes of the samples. If the trained classifier has good accuracy over the test set, then intuitively it means that the joint distribution $f_{X,Y,Z}(.)$ is distinguishable from $f^{CI}$ (note that the generated samples labeled 0 are close in distribution to $f^{CI}$). Therefore, we reject $\mathcal{H}_0$. On the other hand, if the classifier has accuracy close to random guessing, then $f_{X,Y,Z}(.)$ is in fact close to $f^{CI}$, and we fail to reject $\mathcal{H}_0$. 

The advantage of this modular approach is that we can harness the power of classifiers (in step~\ref{step3} above), which have good accuracies in high-dimensions. Binary classification has been used before for two-sample testing in~\cite{lopez2016revisiting}. Therefore, any improvements in the field of binary classification imply an advancement in our CI test. Moreover, there is added flexibility in choosing the best classifiers based on domain knowledge about the data-generation process. Finally, the nearest-neighbor based bootstrap is also efficient owing to fast algorithms for identifying nearest-neighbors~\cite{ramasubramanian1992fast}. 

\subsection{Main Contributions}
\label{contri}
$(i)$ {\bf (Reduction to Classification)} We reduce the problem of CI testing to Binary Classification as detailed in steps~\ref{step1}-\ref{step3} above and in Fig.~\ref{fig:illustrate}. We simulate samples that are close to $f^{CI}$ through a novel nearest-neighbor bootstrap (Algorithm~\ref{alg:NNB}) given access to i.i.d samples from the joint distribution. The problem of CI testing then reduces to a two-sample test between the original samples in $\mathcal{U}$ and $\mathcal{U}'$, which can be effectively done by binary classifiers.

$(ii)$ {\bf (Guarantees on Bootstrapped Samples)} One of our main theoretical results is that the marginal distribution of a sample generated by the nearest-neighbor bootstrap is close in variational distance to the conditionally independent distribution $f^{CI}$. Let $\phi_{X,Y,Z}(x,y,z)$ denote the distribution of a sample produced by Algorithm~\ref{alg:NNB}, when it is supplied with $n$ i.i.d  samples from $f(x,y,z)$. In Theorem~\ref{thm:dtv}, we prove that $d_{TV}(\phi, f^{CI}) = O(1/n^{1/d_z})$ under appropriate smoothness assumptions. Here $d_z$ is the dimension of $Z$ and $d_{TV}$ denotes total variational distance (Def.~\ref{dtv}).

$(iii)$ {\bf (Generalization Bounds for Classification under \textit{near-independence})} The samples generated from the nearest-neighbor bootstrap do not remain i.i.d but they are \textit{close} to i.i.d. We quantify this property and go on to show generalization risk bounds for the classifier. Let us denote the class of function encoded by the classifier as $\mathcal{G}$. Let $\hat{R}$ denote the probability of error of the optimal classifier $\hat{g} \in \mathcal{G}$ trained on the training set (Fig.~\ref{fig:illustrate}). We prove that under appropriate assumptions, we have 
\[ 0.5(1 - d_{TV}(f,f^{CI})) \leq  \hat{R} \leq 0.5(1 - d_{TV}(f,f^{CI})) + O(1/n^{1/d_z}) + O\left(\sqrt{\frac{2^{d_z}V}{n}}\right) \]
with high probability. Here $V$ is the VC dimension~\cite{vapnik2015uniform} of the class $\mathcal{G}$. Thus when $f$ is equivalent to $f^{CI}$ ($\mathcal{H}_0$ holds) then the error rate of the classifier is close to $0.5$. We provide a novel analysis of Rademacher complexity bounds~\cite{boucheron2005theory} under near-independence which is of independent interest. 

$(iv)$ {\bf (Empirical Evaluation)} We perform extensive numerical experiments where our algorithm outperforms the state of the art~\cite{zhang2012kernel,strobl2017approximate}. We also apply our algorithm for analyzing CI relations in the protein signaling network  data from the flow cytometry data-set~\cite{sachs2005causal}. In practice we observe that the performance with respect to dimension of $Z$ scales much better than expected from our worst case theoretical analysis. This is because powerful binary classifiers perform well in high-dimensions. 





















%The main contributions of this paper are as follows:
%
%$(i)$ {\bf (Nearest-Neighbor Bootstrap)} We propose a nearest-neighbor based bootstrap method to produce samples whose distributions are close to $f^{CI}$, given access to $n$ i.i.d samples from the joint $f_{X,Y,Z}(x,y,z)$. This is Algorithm~\ref{alg:NNB} in our paper. We prove that the variational distance between the distribution of any one of the samples returned by Algorithm~\ref{alg:NNB} and $f^{CI}$ (conditionally independent distribution) is $O((1/n)^{1/2d_z})$ under mild smoothness assumptions on $f_{X,Y,Z}(x,y,z)$. 
%
%$(ii)$ {\bf (Reduction to Classification)} We reduce the problem of CI tests into a binary classification problem, through our nearest neighbor bootstrap. As shown in Fig.~\ref{fig:illustrate}, we withhold $n/3$ of the original samples in data-set $\mathcal{U}$, while $2n/3$ of the original samples are passed through the nearest neighbor boot-strap to create $n/3$ samples (in $\mathcal{U}'$), that are close to $f^{CI}$ in distribution.  The samples in $\mathcal{U}$ are labeled $1$ and the ones in $\mathcal{U}'$ are labeled $0$. This labeled data-set is broken into training set $\mathcal{D}_r$ and test set $\mathcal{D}_e$. A classifier $\hat{g}$ is trained on $\mathcal{D}_r$. 
%
%The key idea is that if the original samples are in fact CI ($\mathcal{H}_0$ holds), then the two data-sets cannot be distinguished and the test error $\hat{L}(\hat{g},\mathcal{D}_{e})$ will be close to $0.5$ (random guessing). However, if $\mathcal{H}_1$ holds, then the classifier will be able to differentiate between the data-sets i.e. $\hat{L}(\hat{g},\mathcal{D}_{e}) < 0.5$ would be observed. We provide a detailed pseudo-code in Algorithm~\ref{alg:ccitv1}.
%
%$(iii)$ {\bf (Bias Corrected Algorithm)} We provide an improved algorithm in Algorithm~\ref{alg:ccitv2}. The samples generated in the nearest-neighbor boot-strap are close to $f^{CI}$ but the variational distance is not exactly equal to $0$ for finite $n$. Moreover the bootstrapped samples are not exactly i.i.d. Therefore, the trained classifier is expected to have a bias i.e the classifier can achieve a test loss slightly less than 0.5, even when $\mathcal{H}_0$ holds. In Algorithm~\ref{alg:ccitv2}, we propose a simple idea to rectify this bias.  
%
%%(i) a part of the original i.i.d samples are labeled $1$ (ii) the other part of the original samples are supplied to Algorithm~\ref{alg:NNB} to produce samples that are close to $f^{CI}$. These new samples are labeled $0$. (iii) A subset labeled samples are supplied to a binary classifier for training. The trained classifier is tested on a validation set (separate from the training set). If the trained classifier has good accuracy over a validation set, then intuitively it means that the joint distribution $f_{X,Y,Z}(.)$ is distinguishable from $f^{CI}$ (note that the generated samples labeled 0 are close in distribution to $f^{CI}$). Therefore, we reject $\mathcal{H}_0$. On the other hand, if the classifier has accuracy close to random guessing, then $f_{X,Y,Z}(.)$ is in fact close to $f^{CI}$, and we fail to reject $\mathcal{H}_0$.
%
%$(iv)$ {\bf (Novel Generalization Guarantees for Classification)} The samples generated by the nearest-neighbor bootstrap are not i.i.d any more, but they are \textit{close} to i.i.d. We show that even though these samples are not i.i.d, generalization bounds (similar to~\cite{boucheron2005theory} ) for the risk of classifiers trained on them, still hold. (add details about the result). In proving this, we provide a novel analysis for Rademacher type bounds (refer to ~\cite{boucheron2005theory}) for non-i.i.d samples, which relate the classification accuracy to the number of samples and the $VC$-dimension~\cite{vapnik2015uniform} of the class of functions in the classifier. This analysis technique may be of independent interest. 
%
%$(v)$ {\bf (Empirical Validation)} We perform better on real and simulated data..........need more evidence to write. 
%


==> Introductionv3.tex <==
%Rough Story....
%
%(i) Three areas where CI tests are the main work-horse:
%
%(1) Markov Blanket Estimation with cites.
%
%(2) Bayesian Network Learning - add cites
%
%(3) Causal Structure learning - discuss both constraint based and score based contributions. 
%
%Prior work on parametric and non-parametric CI. Kernel based methods. Discuss run time and dimensionality hit. 
%
%(ii) Discuss that ours is a modular approach- simple bootstrap followed by powerful classifiers. Classifiers can be flexibly chosen with domain knowledge, and any advancement in this field implies an advancement in ours. Discuss dimension issues. 
%
%(iii) List main contributions:
%
%(1) Reduction to classification with NNB.
%
%(2) Guarantees for NNB
%
%(3) Novel guarantees for non-i.i.d classification
%
%(4) Empirical Performance. 

%%%%%%%%%%%%%%%%%%%%%%%%%Start Intro%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
Conditional Independence is a fundamental concept with a wide range of applications in statistics and machine learning~\cite{dawid1979conditional}. Given a set of triplets of random variables $(X, Y, Z)$, we say that $X$ is conditionally independent of $Y$ given $Z$ (denoted by $X \independent Y \vert Z$), when the joint distribution $f_{X,Y,Z}(x,y,z)$ factorizes as $f_{X,Y,Z}(x,y,z) = f_{X|Z}(x|z)f_{Y|Z}(y|z)f_{Z}(z)$. The problem of \textit{Conditional Independence Testing} (CI Testing) can be defined as follows: Given $n$ i.i.d samples from $f_{X,Y,Z}(x,y,z)$, distinguish between the two hypothesis $\mathcal{H}_0:$ $X \independent Y \vert Z$ and $\mathcal{H}_1:$ $X \centernot{\independent} Y \vert Z$. 

CI tests are fundamental tools for learning Bayesian networks~\cite{koller2009probabilistic}, causal inference~\cite{pearl2009causality} and feature selection through Markov Blankets~\cite{koller1996toward}. In causal structure learning, results of CI tests among the nodes of a causal graph~\cite{pearl2009causality} are vital inputs to popular constraint based algorithms~\cite{kalisch2007estimating,tsamardinos2006max}. A key property is that given two variables on a causal graph $X$ and $Y$ and a vector of other variables $Z$ (vector of nodes in the causal graph), $X \independent Y \vert Z$, implies the absence of an edge between $X$ and $Y$. Some of the more recent score-based methods of causal inference also rely on effective CI tests~\cite{brenner2013sparsityboost}. Similarly in the field of learning Bayesian networks, results from CI tests are used to discover edges between random variables that form the nodes of the network~\cite{spirtes2000causation,cheng1998learning,de2000new}. CI tests are also useful in the field of feature selection for high-dimensional supervised learning problems through Markov blankets~\cite{koller1996toward, xing2001feature}. It is important to note that in many of these settings, while $X,Y$ might be low-dimensional, $Z$ is high-dimensional due to the size of the conditioning set that potentially separates $(X,Y)$ from the rest of the graph.

CI testing is fundamentally much harder than testing for independence (i.e whether $X \independent Y$)~\cite{bergsma2004testing}. When $Z$ is discrete, CI tests can be reduced to independence tests by partitioning the data-set according to values of $Z$, and testing for independence separately in each partition. The continuous setting is more difficult, where traditional methods focus on parametric assumptions like linear relations between the random variables with additive Gaussian noise, where the problem reduces to testing for correlations~\cite{lawrance1976conditional}. Our focus is on \textit{non-parametric} CI testing for continuous random variables, i.e. determining CI relations without such simplifying assumptions. 

Some of the earlier methods for non-parametric CI testing, either involve discretizing $Z$ into sets of bins~\cite{margaritis2005distribution}, or involve estimating the marginal densities $f_{X \vert Z}(.)$ and $f_{Y \vert Z}(.)$~\cite{su2007consistent}. Unfortunately, these methods do not perform well in higher dimensions of $Z$. Recently, powerful kernel based methods for non-parametric CI testing have been proposed that are accurate even for moderate values of the dimensions of $Z$~\cite{gao2016demystifying,strobl2017approximate,zhang2012kernel,doran2014permutation}. 
%Many of these approaches are based on the observation in~\cite{fukumizu2004dimensionality}, that non-parametric CI relations can be characterized using covariance operators in the reproducing kernel Hilbert spaces (RKHS). 
However, even these kernel based methods have issues in accuracy of the test when the dimension of the conditioning set is large~\cite{doran2014permutation} and also incur prohibitive running times when the number of samples ($n$) is large~\cite{strobl2017approximate}. 

\begin{figure}[h]
	\centering
	\includegraphics[width=8cm,height=4.5cm]{illustrate.pdf}
	\caption{Illustration of our methodology. A part of the original samples are kept aside in $\mathcal{U}$. The rest of the samples are used in our nearest neighbor boot-strap to generate a data-set $\mathcal{U}'$ which is close to $f^{CI}$ in distribution. The samples are labeled as shown and a classifier is trained on a training set. The test error is measured on a test set there-after. If the test-error is close to $0.5$, then $\mathcal{H}_0$ is not rejected, however if the test error is low then $\mathcal{H}_0$ is rejected.}
	\label{fig:illustrate}
\end{figure}

In this paper, we take a modular approach (illustrated in Fig.~\ref{fig:illustrate}), which reduces the problem of CI testing to Binary Classification~\cite{boucheron2005theory} as follows:

\setword{$(i)$}{step1} For ease of exposition, we assume that we are provided $3n$ i.i.d samples from $f_{X,Y,Z}(x,y,z)$. $n$ of these original samples are kept aside in $\mathcal{U}_1$ (refer to Fig.~\ref{fig:illustrate}). The remaining $2n$ of the original samples are processed through our first module, the nearest-neighbor bootstrap, which produces $n$ simulated samples stored in $\mathcal{U}_2'$. The nearest-neighbor bootstrap is Algorithm~\ref{alg:NNB} in our paper. In Sections~\ref{sec:results}, we show that the generated samples in $\mathcal{U}_2'$ are in fact close in total variational distance (defined in Section~\ref{sec:results}) to the distribution $f^{CI}(x,y,z) \triangleq f_{X|Z}(x|z)f_{Y|Z}(y|z)f_Z(z)$. Note that $f^{CI}(.) = f_{X,Y,Z}(.)$ when $\mathcal{H}_0$ holds.    




%The first module in our method is a Nearest-neighbor based boot-strap which simulates $n/2$ new samples, when supplied with $n$ i.i.d samples from the joint distribution $f_{X,Y,Z}(x,y,z)$. In Sections~\ref{sec:Algorithm} and \ref{sec:results}, we show that these new samples are in fact close in variational distance (defined in Section~\ref{sec:results}) to the distribution $f^{CI}(x,y,z) \triangleq f_{X|Z}(x|z)f_{Y|Z}(y|z)f_Z(z)$. As shown in Fig.~\ref{fig:illustrate}, $n/3$ original samples are kept aside in $\mathcal{U}$, while the remaining $2n/3$ are used to generate $n/3$ samples (close to $f^{CI}$ in distribution) in $\mathcal{U}'$, using our nearest-neighbor bootstrap. 

\setword{$(ii)$}{step2} Subsequently, the original samples kept aside in $\mathcal{U}_1$ are labeled $1$ while the new samples simulated from the nearest-neighbor bootstrap (in $\mathcal{U}_2'$) are labeled $0$. The labeled samples ($\mathcal{U}_1$ with label $1$ and $\mathcal{U}_2'$ labeled 0) are aggregated into a data-set $\mathcal{D}$. $\mathcal{D}$ is then broken into training and test sets $\mathcal{D}_r$ and $\mathcal{D}_e$ each containing $n$ samples each. 

\setword{$(iii)$}{step3} Given the labeled training data-set (from step (ii)), we train powerful classifiers such as gradient boosted trees~\cite{chen2016xgboost} or deep neural networks~\cite{krizhevsky2012imagenet} which attempt to learn the classes of the samples. If the trained classifier has good accuracy over the test set, then intuitively it means that the joint distribution $f_{X,Y,Z}(.)$ is distinguishable from $f^{CI}$ (note that the generated samples labeled 0 are close in distribution to $f^{CI}$). Therefore, we reject $\mathcal{H}_0$. On the other hand, if the classifier has accuracy close to random guessing, then $f_{X,Y,Z}(.)$ is in fact close to $f^{CI}$, and we fail to reject $\mathcal{H}_0$. 

The advantage of this modular approach is that we can harness the power of classifiers (in step~\ref{step3} above), which have good accuracies in high-dimensions. Binary classification has in fact been used recently for two-sample testing in~\cite{lopez2016revisiting}. Thus, any improvements in the field of binary classification imply an advancement in our CI test. Moreover, there is added flexibility in choosing the best classifier based on domain knowledge about the data-generation process. Finally, the nearest-neighbor based bootstrap is also efficient owing to fast algorithms for identifying nearest-neighbors~\cite{ramasubramanian1992fast}. 

\subsection{Main Contributions}
\label{contri}
$(i)$ {\bf (Classification based CI testing)} We reduce the problem of CI testing to Binary Classification as detailed in steps~\ref{step1}-\ref{step3} above and in Fig.~\ref{fig:illustrate}. We simulate samples that are close to $f^{CI}$ through a novel nearest-neighbor bootstrap (Algorithm~\ref{alg:NNB}) given access to i.i.d samples from the joint distribution. The problem of CI testing then reduces to a two-sample test between the original samples in $\mathcal{U}_1$ and $\mathcal{U}_2'$, which can be effectively done by binary classifiers.

$(ii)$ {\bf (Guarantees on Bootstrapped Samples)} As mentioned in steps~\ref{step1}-\ref{step3}, if the samples generated by the bootstrap (in $\mathcal{U}_2'$) are close to $f^{CI}$, then the CI testing problem reduces to testing whether the data-sets $\mathcal{U}_1$ and $\mathcal{U}_2'$ are distinguishable from each other.  We theoretically justify that this is indeed true. Let $\phi_{X,Y,Z}(x,y,z)$ denote the distribution of a sample produced by Algorithm~\ref{alg:NNB}, when it is supplied with $n$ i.i.d  samples from $f(x,y,z)$. In Theorem~\ref{thm:dtv}, we prove that $d_{TV}(\phi, f^{CI}) = O(1/n^{1/d_z})$ under appropriate smoothness assumptions. Here $d_z$ is the dimension of $Z$ and $d_{TV}$ denotes total variational distance (Def.~\ref{dtv}). 

%One of our main theoretical results is that the marginal distribution of a sample generated by the nearest-neighbor bootstrap is close in variational distance to the conditionally independent distribution $f^{CI}$. Let $\phi_{X,Y,Z}(x,y,z)$ denote the distribution of a sample produced by Algorithm~\ref{alg:NNB}, when it is supplied with $n$ i.i.d  samples from $f(x,y,z)$. In Theorem~\ref{thm:dtv}, we prove that $d_{TV}(\phi, f^{CI}) = O(1/n^{1/d_z})$ under appropriate smoothness assumptions. Here $d_z$ is the dimension of $Z$ and $d_{TV}$ denotes total variational distance (Def.~\ref{dtv}).

$(iii)$ {\bf (Generalization Bounds for Classification under \textit{near-independence})} The samples generated from the nearest-neighbor bootstrap do not remain i.i.d but they are \textit{close} to i.i.d. We quantify this property and go on to show generalization risk bounds for the classifier. Let us denote the class of function encoded by the classifier as $\mathcal{G}$. Let $\hat{R}$ denote the probability of error of the optimal classifier $\hat{g} \in \mathcal{G}$ trained on the training set (Fig.~\ref{fig:illustrate}). We prove that under appropriate assumptions, we have 
\begin{align*} &r_{0} - O(1/n^{1/d_z}) \leq  \hat{R}  \leq r_{0} + \mathcal{O}(1/n^{1/d_z}) + \mathcal{O}\left(\sqrt{V} \left( n^{-1/3} + \sqrt{2^{d_z}/n} \right)\right) \end{align*}
with high probability, upto log factors. Here $r_0 = 0.5(1 - d_{TV}(f,f^{CI}))$, $V$ is the VC dimension~\cite{vapnik2015uniform} of the class $\mathcal{G}$.  Thus when $f$ is equivalent to $f^{CI}$ ($\mathcal{H}_0$ holds) then the error rate of the classifier is close to $0.5$. But when $\mathcal{H}_1$ holds the loss is much lower.  We provide a novel analysis of Rademacher complexity bounds~\cite{boucheron2005theory} under near-independence which is of independent interest. 

$(iv)$ {\bf (Empirical Evaluation)} We perform extensive numerical experiments where our algorithm outperforms the state of the art~\cite{zhang2012kernel,strobl2017approximate}. We also apply our algorithm for analyzing CI relations in the protein signaling network  data from the flow cytometry data-set~\cite{sachs2005causal}. In practice we observe that the performance with respect to dimension of $Z$ scales much better than expected from our worst case theoretical analysis. This is because powerful binary classifiers perform well in high-dimensions. 





















%The main contributions of this paper are as follows:
%
%$(i)$ {\bf (Nearest-Neighbor Bootstrap)} We propose a nearest-neighbor based bootstrap method to produce samples whose distributions are close to $f^{CI}$, given access to $n$ i.i.d samples from the joint $f_{X,Y,Z}(x,y,z)$. This is Algorithm~\ref{alg:NNB} in our paper. We prove that the variational distance between the distribution of any one of the samples returned by Algorithm~\ref{alg:NNB} and $f^{CI}$ (conditionally independent distribution) is $O((1/n)^{1/2d_z})$ under mild smoothness assumptions on $f_{X,Y,Z}(x,y,z)$. 
%
%$(ii)$ {\bf (Reduction to Classification)} We reduce the problem of CI tests into a binary classification problem, through our nearest neighbor bootstrap. As shown in Fig.~\ref{fig:illustrate}, we withhold $n/3$ of the original samples in data-set $\mathcal{U}$, while $2n/3$ of the original samples are passed through the nearest neighbor boot-strap to create $n/3$ samples (in $\mathcal{U}'$), that are close to $f^{CI}$ in distribution.  The samples in $\mathcal{U}$ are labeled $1$ and the ones in $\mathcal{U}'$ are labeled $0$. This labeled data-set is broken into training set $\mathcal{D}_r$ and test set $\mathcal{D}_e$. A classifier $\hat{g}$ is trained on $\mathcal{D}_r$. 
%
%The key idea is that if the original samples are in fact CI ($\mathcal{H}_0$ holds), then the two data-sets cannot be distinguished and the test error $\hat{L}(\hat{g},\mathcal{D}_{e})$ will be close to $0.5$ (random guessing). However, if $\mathcal{H}_1$ holds, then the classifier will be able to differentiate between the data-sets i.e. $\hat{L}(\hat{g},\mathcal{D}_{e}) < 0.5$ would be observed. We provide a detailed pseudo-code in Algorithm~\ref{alg:ccitv1}.
%
%$(iii)$ {\bf (Bias Corrected Algorithm)} We provide an improved algorithm in Algorithm~\ref{alg:ccitv2}. The samples generated in the nearest-neighbor boot-strap are close to $f^{CI}$ but the variational distance is not exactly equal to $0$ for finite $n$. Moreover the bootstrapped samples are not exactly i.i.d. Therefore, the trained classifier is expected to have a bias i.e the classifier can achieve a test loss slightly less than 0.5, even when $\mathcal{H}_0$ holds. In Algorithm~\ref{alg:ccitv2}, we propose a simple idea to rectify this bias.  
%
%%(i) a part of the original i.i.d samples are labeled $1$ (ii) the other part of the original samples are supplied to Algorithm~\ref{alg:NNB} to produce samples that are close to $f^{CI}$. These new samples are labeled $0$. (iii) A subset labeled samples are supplied to a binary classifier for training. The trained classifier is tested on a validation set (separate from the training set). If the trained classifier has good accuracy over a validation set, then intuitively it means that the joint distribution $f_{X,Y,Z}(.)$ is distinguishable from $f^{CI}$ (note that the generated samples labeled 0 are close in distribution to $f^{CI}$). Therefore, we reject $\mathcal{H}_0$. On the other hand, if the classifier has accuracy close to random guessing, then $f_{X,Y,Z}(.)$ is in fact close to $f^{CI}$, and we fail to reject $\mathcal{H}_0$.
%
%$(iv)$ {\bf (Novel Generalization Guarantees for Classification)} The samples generated by the nearest-neighbor bootstrap are not i.i.d any more, but they are \textit{close} to i.i.d. We show that even though these samples are not i.i.d, generalization bounds (similar to~\cite{boucheron2005theory} ) for the risk of classifiers trained on them, still hold. (add details about the result). In proving this, we provide a novel analysis for Rademacher type bounds (refer to ~\cite{boucheron2005theory}) for non-i.i.d samples, which relate the classification accuracy to the number of samples and the $VC$-dimension~\cite{vapnik2015uniform} of the class of functions in the classifier. This analysis technique may be of independent interest. 
%
%$(v)$ {\bf (Empirical Validation)} We perform better on real and simulated data..........need more evidence to write. 
%


==> Introductionv4.tex <==
%Rough Story....
%
%(i) Three areas where CI tests are the main work-horse:
%
%(1) Markov Blanket Estimation with cites.
%
%(2) Bayesian Network Learning - add cites
%
%(3) Causal Structure learning - discuss both constraint based and score based contributions. 
%
%Prior work on parametric and non-parametric CI. Kernel based methods. Discuss run time and dimensionality hit. 
%
%(ii) Discuss that ours is a modular approach- simple bootstrap followed by powerful classifiers. Classifiers can be flexibly chosen with domain knowledge, and any advancement in this field implies an advancement in ours. Discuss dimension issues. 
%
%(iii) List main contributions:
%
%(1) Reduction to classification with NNB.
%
%(2) Guarantees for NNB
%
%(3) Novel guarantees for non-i.i.d classification
%
%(4) Empirical Performance. 

%%%%%%%%%%%%%%%%%%%%%%%%%Start Intro%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
Conditional Independence is a fundamental concept with a wide range of applications in statistics and machine learning~\cite{dawid1979conditional}. Given a set of triplets of random variables $(X, Y, Z)$, we say that $X$ is conditionally independent of $Y$ given $Z$ (denoted by $X \independent Y \vert Z$), when the joint distribution $f_{X,Y,Z}(x,y,z)$ factorizes as $f_{X,Y,Z}(x,y,z) = f_{X|Z}(x|z)f_{Y|Z}(y|z)f_{Z}(z)$. The problem of \textit{Conditional Independence Testing} (CI Testing) can be defined as follows: Given $n$ i.i.d samples from $f_{X,Y,Z}(x,y,z)$, distinguish between the two hypothesis $\mathcal{H}_0:$ $X \independent Y \vert Z$ and $\mathcal{H}_1:$ $X \centernot{\independent} Y \vert Z$. 

CI tests are fundamental tools for learning Bayesian networks~\cite{koller2009probabilistic}, causal inference~\cite{pearl2009causality} and feature selection through Markov Blankets~\cite{koller1996toward}. In causal structure learning, results of CI tests among the nodes of a causal graph~\cite{pearl2009causality} are vital inputs to popular constraint based algorithms~\cite{kalisch2007estimating,tsamardinos2006max}. A key property is that given two variables on a causal graph $X$ and $Y$ and a vector of other variables $Z$ (vector of nodes in the causal graph), $X \independent Y \vert Z$, implies the absence of an edge between $X$ and $Y$. Some of the more recent score-based methods of causal inference also rely on effective CI tests~\cite{brenner2013sparsityboost}. Similarly in the field of learning Bayesian networks, results from CI tests are used to discover edges between random variables that form the nodes of the network~\cite{spirtes2000causation,cheng1998learning,de2000new}. CI tests are also useful in the field of feature selection for high-dimensional supervised learning problems through Markov blankets~\cite{koller1996toward, xing2001feature}. It is important to note that in many of these settings, while $X,Y$ might be low-dimensional, $Z$ is high-dimensional due to the size of the conditioning set that potentially separates $(X,Y)$ from the rest of the graph.

In this paper we propose a data-driven \textit{Model-powered} test: instead of computing some statistic or using an analytical approach, we convert 
the conditional independence question into something a model (a classifier or regressor) can answer by \textit{training on data}. 
This allows us to harness the ability of modern powerful models (like gradient-boosted trees and deep neural networks) to extract information from high-dimensional datasets.

Our approach is inspired by Classifier Two-Sample tests~\cite{LopezPaz,OthersBBB} which use this approach for independence testing and two-sample tests.  
We start by understanding how to build a model-powered independence test.
For two random variables $X,Y$ we are given i.i.d. samples $(X_i,Y_i)$, $i=1 \ldots n/2$ and we would like to know if $X$ is independent from $Y$.
To achieve this, we split the samples in half: for the first half simply add the label $y=0$ for $i=1 \ldots n/2$, indicating unshuffled data. For the other half, we randomly permute $Y_i$, i.e. create $(X_i, Y_{\pi (i)})$, $i= n/2, \ldots n$, for a random permutation $\pi(i)$ and add the label $Y=1$, i.e. mark them as shuffled. 
Now we give half of the shuffled and half the unshuffled data to a classifier that tries to learn to predict if a tuple is shuffled, or not. 
We can subsequently use the remaining data to test the model accuracy. If the model can confidently distinguish between shuffled and un-shuffled $(X_i,Y_i)$ tuples, this proves that $X$ and $Y$ are not independent. Note that, as usual, we can never confidently show that $X$ and $Y$ \textit{are} independent since our model may be weak and fail to capture some complex dependency structure between $X$ and $Y$. For this reason we can confidently reject (or fail to reject) the independence Null hypothesis and $p$-values can be easily obtained since the model would be performing random guesses under the Null. 

Conditional independence testing is fundamentally harder than independence testing (see e.g.~\cite{bergsma2004testing}). When $Z$ is discrete, CI tests can be reduced to multiple independence tests, one for each value of $Z$. The continuous setting is more challenging
and previous methods often rely on parametric assumptions like linear relations between the random variables with additive Gaussian noise, where the problem reduces to testing for correlations~\cite{lawrance1976conditional}. Our focus is on \textit{non-parametric} CI testing for continuous random variables, i.e. determining CI relations under minimal simplifying assumptions. 

Some of the earlier methods for non-parametric CI testing, either involve discretizing $Z$ into sets of bins~\cite{margaritis2005distribution}, or involve estimating the marginal densities $f_{X \vert Z}(.)$ and $f_{Y \vert Z}(.)$~\cite{su2007consistent}. Unfortunately, these methods do not perform well in higher dimensions of $Z$. Recently, powerful kernel based methods for non-parametric CI testing have been proposed that are accurate even for moderate values of the dimensions of $Z$~\cite{gao2016demystifying,strobl2017approximate,zhang2012kernel,doran2014permutation}. 
%Many of these approaches are based on the observation in~\cite{fukumizu2004dimensionality}, that non-parametric CI relations can be characterized using covariance operators in the reproducing kernel Hilbert spaces (RKHS). 
However, even these kernel based methods have issues in accuracy of the test when the dimension of the conditioning set is large~\cite{doran2014permutation} and also incur prohibitive running times when the number of samples ($n$) is large~\cite{strobl2017approximate}. 

\begin{figure}[h]
	\centering
	\includegraphics[width=8cm,height=4.5cm]{illustrate.pdf}
	\caption{Illustration of our methodology. A part of the original samples are kept aside in $\mathcal{U}$. The rest of the samples are used in our nearest neighbor boot-strap to generate a data-set $\mathcal{U}'$ which is close to $f^{CI}$ in distribution. The samples are labeled as shown and a classifier is trained on a training set. The test error is measured on a test set there-after. If the test-error is close to $0.5$, then $\mathcal{H}_0$ is not rejected, however if the test error is low then $\mathcal{H}_0$ is rejected.}
	\label{fig:illustrate}
\end{figure}

In this paper, we take a modular approach (illustrated in Fig.~\ref{fig:illustrate}), which reduces the problem of CI testing to Binary Classification.
For vanilla independence testing, the key property was that the permuted tuples  $(X_i,Y_{\pi(i)})$ are i.i.d. samples from the product distribution 
density $f(x)f(y)$. It is quite interesting that a permutation allows us create samples from $f(x)f(y)$ without needing to learn these potentially high-dimensional distributions.  To perform conditional independence tests we have to solve the analogous problem: we need to create samples from the conditional product distribution  $f^{CI}(x,y,z) = f(x|z)f(y|z)f(z)$, given access only to i.i.d.
samples from the joint distribution $f(x,y,z)$.
Our key technical contribution is to show how this can be done with a nearest-neighbor bootstrap procedure and establish 
that these are close in total variation distance to the true $f^{CI}$ distribution. 
 
Specifically, the steps of our algorithm are: 
\setword{$(i)$}{step1} For ease of exposition, we assume that we are provided $3n$ i.i.d samples from $f_{X,Y,Z}(x,y,z)$. $n$ of these original samples are kept aside in $\mathcal{U}_1$ (refer to Fig.~\ref{fig:illustrate}). The remaining $2n$ of the original samples are processed through our first module, the nearest-neighbor bootstrap, which produces $n$ simulated samples stored in $\mathcal{U}_2'$. The nearest-neighbor bootstrap is Algorithm~\ref{alg:NNB} in our paper. In Sections~\ref{sec:results}, we show that the generated samples in $\mathcal{U}_2'$ are in fact close in total variational distance (defined in Section~\ref{sec:results}) to the distribution $f^{CI}(x,y,z) \triangleq f_{X|Z}(x|z)f_{Y|Z}(y|z)f_Z(z)$. Note that $f^{CI}(.) = f_{X,Y,Z}(.)$ when $\mathcal{H}_0$ holds.    




%The first module in our method is a Nearest-neighbor based boot-strap which simulates $n/2$ new samples, when supplied with $n$ i.i.d samples from the joint distribution $f_{X,Y,Z}(x,y,z)$. In Sections~\ref{sec:Algorithm} and \ref{sec:results}, we show that these new samples are in fact close in variational distance (defined in Section~\ref{sec:results}) to the distribution $f^{CI}(x,y,z) \triangleq f_{X|Z}(x|z)f_{Y|Z}(y|z)f_Z(z)$. As shown in Fig.~\ref{fig:illustrate}, $n/3$ original samples are kept aside in $\mathcal{U}$, while the remaining $2n/3$ are used to generate $n/3$ samples (close to $f^{CI}$ in distribution) in $\mathcal{U}'$, using our nearest-neighbor bootstrap. 

\setword{$(ii)$}{step2} Subsequently, the original samples kept aside in $\mathcal{U}_1$ are labeled $1$ while the new samples simulated from the nearest-neighbor bootstrap (in $\mathcal{U}_2'$) are labeled $0$. The labeled samples ($\mathcal{U}_1$ with label $1$ and $\mathcal{U}_2'$ labeled 0) are aggregated into a data-set $\mathcal{D}$. $\mathcal{D}$ is then broken into training and test sets $\mathcal{D}_r$ and $\mathcal{D}_e$ each containing $n$ samples each. 

\setword{$(iii)$}{step3} Given the labeled training data-set (from step (ii)), we train powerful classifiers such as gradient boosted trees~\cite{chen2016xgboost} or deep neural networks~\cite{krizhevsky2012imagenet} which attempt to learn the classes of the samples. If the trained classifier has good accuracy over the test set, then intuitively it means that the joint distribution $f_{X,Y,Z}(.)$ is distinguishable from $f^{CI}$ (note that the generated samples labeled 0 are close in distribution to $f^{CI}$). Therefore, we reject $\mathcal{H}_0$. On the other hand, if the classifier has accuracy close to random guessing, then $f_{X,Y,Z}(.)$ is in fact close to $f^{CI}$, and we fail to reject $\mathcal{H}_0$. 

The advantage of this modular approach is that we can harness the power of classifiers (in step~\ref{step3} above), which have good accuracies in high-dimensions. Binary classification has in fact been used recently for two-sample testing in~\cite{lopez2016revisiting}. Thus, any improvements in the field of binary classification imply an advancement in our CI test. Moreover, there is added flexibility in choosing the best classifier based on domain knowledge about the data-generation process. Finally, the nearest-neighbor based bootstrap is also efficient owing to fast algorithms for identifying nearest-neighbors~\cite{ramasubramanian1992fast}. 

\subsection{Main Contributions}
\label{contri}
$(i)$ {\bf (Classification based CI testing)} We reduce the problem of CI testing to Binary Classification as detailed in steps~\ref{step1}-\ref{step3} above and in Fig.~\ref{fig:illustrate}. We simulate samples that are close to $f^{CI}$ through a novel nearest-neighbor bootstrap (Algorithm~\ref{alg:NNB}) given access to i.i.d samples from the joint distribution. The problem of CI testing then reduces to a two-sample test between the original samples in $\mathcal{U}_1$ and $\mathcal{U}_2'$, which can be effectively done by binary classifiers.

$(ii)$ {\bf (Guarantees on Bootstrapped Samples)} As mentioned in steps~\ref{step1}-\ref{step3}, if the samples generated by the bootstrap (in $\mathcal{U}_2'$) are close to $f^{CI}$, then the CI testing problem reduces to testing whether the data-sets $\mathcal{U}_1$ and $\mathcal{U}_2'$ are distinguishable from each other.  We theoretically justify that this is indeed true. Let $\phi_{X,Y,Z}(x,y,z)$ denote the distribution of a sample produced by Algorithm~\ref{alg:NNB}, when it is supplied with $n$ i.i.d  samples from $f(x,y,z)$. In Theorem~\ref{thm:dtv}, we prove that $d_{TV}(\phi, f^{CI}) = O(1/n^{1/d_z})$ under appropriate smoothness assumptions. Here $d_z$ is the dimension of $Z$ and $d_{TV}$ denotes total variational distance (Def.~\ref{dtv}). 

%One of our main theoretical results is that the marginal distribution of a sample generated by the nearest-neighbor bootstrap is close in variational distance to the conditionally independent distribution $f^{CI}$. Let $\phi_{X,Y,Z}(x,y,z)$ denote the distribution of a sample produced by Algorithm~\ref{alg:NNB}, when it is supplied with $n$ i.i.d  samples from $f(x,y,z)$. In Theorem~\ref{thm:dtv}, we prove that $d_{TV}(\phi, f^{CI}) = O(1/n^{1/d_z})$ under appropriate smoothness assumptions. Here $d_z$ is the dimension of $Z$ and $d_{TV}$ denotes total variational distance (Def.~\ref{dtv}).

$(iii)$ {\bf (Generalization Bounds for Classification under \textit{near-independence})} The samples generated from the nearest-neighbor bootstrap do not remain i.i.d but they are \textit{close} to i.i.d. We quantify this property and go on to show generalization risk bounds for the classifier. Let us denote the class of function encoded by the classifier as $\mathcal{G}$. Let $\hat{R}$ denote the probability of error of the optimal classifier $\hat{g} \in \mathcal{G}$ trained on the training set (Fig.~\ref{fig:illustrate}). We prove that under appropriate assumptions, we have 
\begin{align*} &r_{0} - O(1/n^{1/d_z}) \leq  \hat{R}  \leq r_{0} + \mathcal{O}(1/n^{1/d_z}) + \mathcal{O}\left(\sqrt{V} \left( n^{-1/3} + \sqrt{2^{d_z}/n} \right)\right) \end{align*}
with high probability, upto log factors. Here $r_0 = 0.5(1 - d_{TV}(f,f^{CI}))$, $V$ is the VC dimension~\cite{vapnik2015uniform} of the class $\mathcal{G}$.  Thus when $f$ is equivalent to $f^{CI}$ ($\mathcal{H}_0$ holds) then the error rate of the classifier is close to $0.5$. But when $\mathcal{H}_1$ holds the loss is much lower.  We provide a novel analysis of Rademacher complexity bounds~\cite{boucheron2005theory} under near-independence which is of independent interest. 

$(iv)$ {\bf (Empirical Evaluation)} We perform extensive numerical experiments where our algorithm outperforms the state of the art~\cite{zhang2012kernel,strobl2017approximate}. We also apply our algorithm for analyzing CI relations in the protein signaling network  data from the flow cytometry data-set~\cite{sachs2005causal}. In practice we observe that the performance with respect to dimension of $Z$ scales much better than expected from our worst case theoretical analysis. This is because powerful binary classifiers perform well in high-dimensions. 





















%The main contributions of this paper are as follows:
%
%$(i)$ {\bf (Nearest-Neighbor Bootstrap)} We propose a nearest-neighbor based bootstrap method to produce samples whose distributions are close to $f^{CI}$, given access to $n$ i.i.d samples from the joint $f_{X,Y,Z}(x,y,z)$. This is Algorithm~\ref{alg:NNB} in our paper. We prove that the variational distance between the distribution of any one of the samples returned by Algorithm~\ref{alg:NNB} and $f^{CI}$ (conditionally independent distribution) is $O((1/n)^{1/2d_z})$ under mild smoothness assumptions on $f_{X,Y,Z}(x,y,z)$. 
%
%$(ii)$ {\bf (Reduction to Classification)} We reduce the problem of CI tests into a binary classification problem, through our nearest neighbor bootstrap. As shown in Fig.~\ref{fig:illustrate}, we withhold $n/3$ of the original samples in data-set $\mathcal{U}$, while $2n/3$ of the original samples are passed through the nearest neighbor boot-strap to create $n/3$ samples (in $\mathcal{U}'$), that are close to $f^{CI}$ in distribution.  The samples in $\mathcal{U}$ are labeled $1$ and the ones in $\mathcal{U}'$ are labeled $0$. This labeled data-set is broken into training set $\mathcal{D}_r$ and test set $\mathcal{D}_e$. A classifier $\hat{g}$ is trained on $\mathcal{D}_r$. 
%
%The key idea is that if the original samples are in fact CI ($\mathcal{H}_0$ holds), then the two data-sets cannot be distinguished and the test error $\hat{L}(\hat{g},\mathcal{D}_{e})$ will be close to $0.5$ (random guessing). However, if $\mathcal{H}_1$ holds, then the classifier will be able to differentiate between the data-sets i.e. $\hat{L}(\hat{g},\mathcal{D}_{e}) < 0.5$ would be observed. We provide a detailed pseudo-code in Algorithm~\ref{alg:ccitv1}.
%
%$(iii)$ {\bf (Bias Corrected Algorithm)} We provide an improved algorithm in Algorithm~\ref{alg:ccitv2}. The samples generated in the nearest-neighbor boot-strap are close to $f^{CI}$ but the variational distance is not exactly equal to $0$ for finite $n$. Moreover the bootstrapped samples are not exactly i.i.d. Therefore, the trained classifier is expected to have a bias i.e the classifier can achieve a test loss slightly less than 0.5, even when $\mathcal{H}_0$ holds. In Algorithm~\ref{alg:ccitv2}, we propose a simple idea to rectify this bias.  
%
%%(i) a part of the original i.i.d samples are labeled $1$ (ii) the other part of the original samples are supplied to Algorithm~\ref{alg:NNB} to produce samples that are close to $f^{CI}$. These new samples are labeled $0$. (iii) A subset labeled samples are supplied to a binary classifier for training. The trained classifier is tested on a validation set (separate from the training set). If the trained classifier has good accuracy over a validation set, then intuitively it means that the joint distribution $f_{X,Y,Z}(.)$ is distinguishable from $f^{CI}$ (note that the generated samples labeled 0 are close in distribution to $f^{CI}$). Therefore, we reject $\mathcal{H}_0$. On the other hand, if the classifier has accuracy close to random guessing, then $f_{X,Y,Z}(.)$ is in fact close to $f^{CI}$, and we fail to reject $\mathcal{H}_0$.
%
%$(iv)$ {\bf (Novel Generalization Guarantees for Classification)} The samples generated by the nearest-neighbor bootstrap are not i.i.d any more, but they are \textit{close} to i.i.d. We show that even though these samples are not i.i.d, generalization bounds (similar to~\cite{boucheron2005theory} ) for the risk of classifiers trained on them, still hold. (add details about the result). In proving this, we provide a novel analysis for Rademacher type bounds (refer to ~\cite{boucheron2005theory}) for non-i.i.d samples, which relate the classification accuracy to the number of samples and the $VC$-dimension~\cite{vapnik2015uniform} of the class of functions in the classifier. This analysis technique may be of independent interest. 
%
%$(v)$ {\bf (Empirical Validation)} We perform better on real and simulated data..........need more evidence to write. 
%


==> Introductionv5.tex <==
%Rough Story....
%
%(i) Three areas where CI tests are the main work-horse:
%
%(1) Markov Blanket Estimation with cites.
%
%(2) Bayesian Network Learning - add cites
%
%(3) Causal Structure learning - discuss both constraint based and score based contributions. 
%
%Prior work on parametric and non-parametric CI. Kernel based methods. Discuss run time and dimensionality hit. 
%
%(ii) Discuss that ours is a modular approach- simple bootstrap followed by powerful classifiers. Classifiers can be flexibly chosen with domain knowledge, and any advancement in this field implies an advancement in ours. Discuss dimension issues. 
%
%(iii) List main contributions:
%
%(1) Reduction to classification with NNB.
%
%(2) Guarantees for NNB
%
%(3) Novel guarantees for non-i.i.d classification
%
%(4) Empirical Performance. 

%%%%%%%%%%%%%%%%%%%%%%%%%Start Intro%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
Testing datasets for conditional independence have significant
applications in several statistical/learning applications; among
others, examples include discovering/testing for edges in Bayesian
networks~\cite{koller2009probabilistic,
  spirtes2000causation,cheng1998learning,de2000new}, causal
inference~\cite{pearl2009causality,
  kalisch2007estimating,tsamardinos2006max, brenner2013sparsityboost}
and feature selection through Markov
Blankets~\cite{koller1996toward,xing2001feature}. Given a set of
triplets of random variables $(X, Y, Z)$, we say that $X$ is
conditionally independent of $Y$ given $Z$ (denoted by
$X \independent Y \vert Z$), if the joint distribution
$f_{X,Y,Z}(x,y,z)$ factorizes as
$f_{X,Y,Z}(x,y,z) = f_{X|Z}(x|z)f_{Y|Z}(y|z)f_{Z}(z)$. The problem of
\textit{Conditional Independence Testing} (CI Testing) can be defined
as follows: Given $n$ i.i.d samples from $f_{X,Y,Z}(x,y,z)$,
distinguish between the two hypothesis $\mathcal{H}_0:$
$X \independent Y \vert Z$ and $\mathcal{H}_1:$
$X \centernot{\independent} Y \vert Z$.

% CI tests are fundamental tools for learning Bayesian
% networks~\cite{koller2009probabilistic}, causal
% inference~\cite{pearl2009causality} and feature selection through
% Markov Blankets~\cite{koller1996toward}. In causal structure learning,
% results of CI tests among the nodes of a causal
% graph~\cite{pearl2009causality} are vital inputs to popular constraint
% based algorithms~\cite{kalisch2007estimating,tsamardinos2006max}. A
% key property is that given two variables on a causal graph $X$ and $Y$
% and a vector of other variables $Z$ (vector of nodes in the causal
% graph), $X \independent Y \vert Z$, implies the absence of an edge
% between $X$ and $Y$. Some of the more recent score-based methods of
% causal inference also rely on effective CI
% tests~\cite{brenner2013sparsityboost}. Similarly in the field of
% learning Bayesian networks, results from CI tests are used to discover
% edges between random variables that form the nodes of the
% network~\cite{spirtes2000causation,cheng1998learning,de2000new}. CI
% tests are also useful in the field of feature selection for
% high-dimensional supervised learning problems through Markov
% blankets~\cite{koller1996toward, xing2001feature}. 


% It is important to note that in many of these settings, while $X,Y$
% might be low-dimensional, $Z$ is high-dimensional due to the size of
% the conditioning set that potentially separates $(X,Y)$ from the rest
% of the graph.

In this paper we propose a data-driven \textit{Model-powered} test:
instead of computing some statistic or using an analytical approach,
we convert the conditional independence question into something a
model (a classifier or regressor) can answer by \textit{training on
  data}. This allows us to harness the ability of modern powerful
models (like gradient-boosted trees and deep neural networks) to
extract information from high-dimensional datasets.

Our approach is inspired by Classifier Two-Sample
tests~\cite{LopezPaz,OthersBBB} which use this approach for
independence testing and two-sample tests. We start by understanding
how to build a model-powered independence test. For two random
variables $X,Y$ we are given i.i.d. samples $(X_i,Y_i)$,
$i=1 \ldots n/2$ and we would like to know if $X$ is independent from
$Y$. To achieve this, we split the samples in half: for the first half
simply add the label $y=0$ for $i=1 \ldots n/2$, indicating unshuffled
data. For the other half, we randomly permute $Y_i$, i.e. create
$(X_i, Y_{\pi (i)})$, $i= n/2, \ldots n$, for a random permutation
$\pi(i)$ and add the label $Y=1$, i.e. mark them as shuffled. Now we
give half of the shuffled and half the unshuffled data to a classifier
that tries to learn to predict if a tuple is shuffled, or not. We can
subsequently use the remaining data to test the model accuracy. If the
model can confidently distinguish between shuffled and un-shuffled
$(X_i,Y_i)$ tuples, this proves that $X$ and $Y$ are not independent.
Note that, as usual, we can never confidently show that $X$ and $Y$
\textit{are} independent since our model may be weak and fail to
capture some complex dependency structure between $X$ and $Y$. For
this reason we can confidently reject (or fail to reject) the
independence Null hypothesis and $p$-values can be easily obtained
since the model would be performing random guesses under the Null.

Conditional independence testing is fundamentally harder than
independence testing (see e.g.~\cite{bergsma2004testing}). When $Z$ is
discrete, CI tests can be reduced to multiple independence tests, one
for each value of $Z$. The continuous setting is more challenging and
previous methods often rely on parametric assumptions like linear
relations between the random variables with additive Gaussian noise,
where the problem reduces to testing for
correlations~\cite{lawrance1976conditional}. Our focus is on
\textit{non-parametric} CI testing for continuous random variables,
i.e. determining CI relations under minimal simplifying assumptions.

Some of the earlier methods for non-parametric CI testing, either
involve discretizing $Z$ into sets of
bins~\cite{margaritis2005distribution}, or involve estimating the
marginal densities $f_{X \vert Z}(.)$ and
$f_{Y \vert Z}(.)$~\cite{su2007consistent}. Unfortunately, these
methods do not perform well in higher dimensions of $Z$. Recently,
powerful kernel based methods for non-parametric CI testing have been
proposed that are accurate even for moderate values of the dimensions
of
$Z$~\cite{gao2016demystifying,strobl2017approximate,zhang2012kernel,doran2014permutation}.
% Many of these approaches are based on the observation
% in~\cite{fukumizu2004dimensionality}, that non-parametric CI
% relations can be characterized using covariance operators in the
% reproducing kernel Hilbert spaces (RKHS).
However, even these kernel based methods have issues in accuracy of
the test when the dimension of the conditioning set is
large~\cite{doran2014permutation} and also incur prohibitive running
times when the number of samples ($n$) is
large~\cite{strobl2017approximate}.

\begin{figure}[h] \centering
  \includegraphics[width=8cm,height=4.5cm]{illustrate.pdf}
  \caption{Illustration of our methodology. A part of the original
    samples are kept aside in $\mathcal{U}$. The rest of the samples
    are used in our nearest neighbor boot-strap to generate a data-set
    $\mathcal{U}'$ which is close to $f^{CI}$ in distribution. The
    samples are labeled as shown and a classifier is trained on a
    training set. The test error is measured on a test set
    there-after. If the test-error is close to $0.5$, then
    $\mathcal{H}_0$ is not rejected, however if the test error is low
    then $\mathcal{H}_0$ is rejected.}
	\label{fig:illustrate}
\end{figure}

In this paper, we take a modular approach (illustrated in
Fig.~\ref{fig:illustrate}), which reduces the problem of CI testing to
Binary Classification. For vanilla independence testing, the key
property was that the permuted tuples $(X_i,Y_{\pi(i)})$ are i.i.d.
samples from the product distribution density $f(x)f(y)$. It is quite
interesting that a permutation allows us create samples from
$f(x)f(y)$ without needing to learn these potentially high-dimensional
distributions. To perform conditional independence tests we have to
solve the analogous problem: we need to create samples from the
conditional product distribution $f^{CI}(x,y,z) = f(x|z)f(y|z)f(z)$,
given access only to i.i.d. samples from the joint distribution
$f(x,y,z)$. Our key technical contribution is to show how this can be
done with a nearest-neighbor bootstrap procedure and establish that
these are close in total variation distance to the true $f^{CI}$
distribution.
 
Specifically, the steps of our algorithm are: \setword{$(i)$}{step1}
For ease of exposition, we assume that we are provided $3n$ i.i.d
samples from $f_{X,Y,Z}(x,y,z)$. $n$ of these original samples are
kept aside in $\mathcal{U}_1$ (refer to Fig.~\ref{fig:illustrate}).
The remaining $2n$ of the original samples are processed through our
first module, the nearest-neighbor bootstrap, which produces $n$
simulated samples stored in $\mathcal{U}_2'$. The nearest-neighbor
bootstrap is Algorithm~\ref{alg:NNB} in our paper. In
Sections~\ref{sec:results}, we show that the generated samples in
$\mathcal{U}_2'$ are in fact close in total variational distance
(defined in Section~\ref{sec:results}) to the distribution
$f^{CI}(x,y,z) \triangleq f_{X|Z}(x|z)f_{Y|Z}(y|z)f_Z(z)$. Note that
$f^{CI}(.) = f_{X,Y,Z}(.)$ when $\mathcal{H}_0$ holds.




% The first module in our method is a Nearest-neighbor based
% boot-strap which simulates $n/2$ new samples, when supplied with $n$
% i.i.d samples from the joint distribution $f_{X,Y,Z}(x,y,z)$. In
% Sections~\ref{sec:Algorithm} and \ref{sec:results}, we show that
% these new samples are in fact close in variational distance (defined
% in Section~\ref{sec:results}) to the distribution
% $f^{CI}(x,y,z) \triangleq f_{X|Z}(x|z)f_{Y|Z}(y|z)f_Z(z)$. As shown
% in Fig.~\ref{fig:illustrate}, $n/3$ original samples are kept aside
% in $\mathcal{U}$, while the remaining $2n/3$ are used to generate
% $n/3$ samples (close to $f^{CI}$ in distribution) in $\mathcal{U}'$,
% using our nearest-neighbor bootstrap.

\setword{$(ii)$}{step2} Subsequently, the original samples kept aside
in $\mathcal{U}_1$ are labeled $1$ while the new samples simulated
from the nearest-neighbor bootstrap (in $\mathcal{U}_2'$) are labeled
$0$. The labeled samples ($\mathcal{U}_1$ with label $1$ and
$\mathcal{U}_2'$ labeled 0) are aggregated into a data-set
$\mathcal{D}$. $\mathcal{D}$ is then broken into training and test
sets $\mathcal{D}_r$ and $\mathcal{D}_e$ each containing $n$ samples
each.

\setword{$(iii)$}{step3} Given the labeled training data-set (from
step (ii)), we train powerful classifiers such as gradient boosted
trees~\cite{chen2016xgboost} or deep neural
networks~\cite{krizhevsky2012imagenet} which attempt to learn the
classes of the samples. If the trained classifier has good accuracy
over the test set, then intuitively it means that the joint
distribution $f_{X,Y,Z}(.)$ is distinguishable from $f^{CI}$ (note
that the generated samples labeled 0 are close in distribution to
$f^{CI}$). Therefore, we reject $\mathcal{H}_0$. On the other hand, if
the classifier has accuracy close to random guessing, then
$f_{X,Y,Z}(.)$ is in fact close to $f^{CI}$, and we fail to reject
$\mathcal{H}_0$.

The advantage of this modular approach is that we can harness the power of classifiers (in step~\ref{step3} above), which have good accuracies in high-dimensions. Binary classification has in fact been used recently for two-sample testing in~\cite{lopez2016revisiting}. Thus, any improvements in the field of binary classification imply an advancement in our CI test. Moreover, there is added flexibility in choosing the best classifier based on domain knowledge about the data-generation process. Finally, the nearest-neighbor based bootstrap is also efficient owing to fast algorithms for identifying nearest-neighbors~\cite{ramasubramanian1992fast}. 

\subsection{Main Contributions}
\label{contri}
$(i)$ {\bf (Classification based CI testing)} We reduce the problem of CI testing to Binary Classification as detailed in steps~\ref{step1}-\ref{step3} above and in Fig.~\ref{fig:illustrate}. We simulate samples that are close to $f^{CI}$ through a novel nearest-neighbor bootstrap (Algorithm~\ref{alg:NNB}) given access to i.i.d samples from the joint distribution. The problem of CI testing then reduces to a two-sample test between the original samples in $\mathcal{U}_1$ and $\mathcal{U}_2'$, which can be effectively done by binary classifiers.

$(ii)$ {\bf (Guarantees on Bootstrapped Samples)} As mentioned in steps~\ref{step1}-\ref{step3}, if the samples generated by the bootstrap (in $\mathcal{U}_2'$) are close to $f^{CI}$, then the CI testing problem reduces to testing whether the data-sets $\mathcal{U}_1$ and $\mathcal{U}_2'$ are distinguishable from each other.  We theoretically justify that this is indeed true. Let $\phi_{X,Y,Z}(x,y,z)$ denote the distribution of a sample produced by Algorithm~\ref{alg:NNB}, when it is supplied with $n$ i.i.d  samples from $f(x,y,z)$. In Theorem~\ref{thm:dtv}, we prove that $d_{TV}(\phi, f^{CI}) = O(1/n^{1/d_z})$ under appropriate smoothness assumptions. Here $d_z$ is the dimension of $Z$ and $d_{TV}$ denotes total variational distance (Def.~\ref{dtv}). 

%One of our main theoretical results is that the marginal distribution of a sample generated by the nearest-neighbor bootstrap is close in variational distance to the conditionally independent distribution $f^{CI}$. Let $\phi_{X,Y,Z}(x,y,z)$ denote the distribution of a sample produced by Algorithm~\ref{alg:NNB}, when it is supplied with $n$ i.i.d  samples from $f(x,y,z)$. In Theorem~\ref{thm:dtv}, we prove that $d_{TV}(\phi, f^{CI}) = O(1/n^{1/d_z})$ under appropriate smoothness assumptions. Here $d_z$ is the dimension of $Z$ and $d_{TV}$ denotes total variational distance (Def.~\ref{dtv}).

$(iii)$ {\bf (Generalization Bounds for Classification under \textit{near-independence})} The samples generated from the nearest-neighbor bootstrap do not remain i.i.d but they are \textit{close} to i.i.d. We quantify this property and go on to show generalization risk bounds for the classifier. Let us denote the class of function encoded by the classifier as $\mathcal{G}$. Let $\hat{R}$ denote the probability of error of the optimal classifier $\hat{g} \in \mathcal{G}$ trained on the training set (Fig.~\ref{fig:illustrate}). We prove that under appropriate assumptions, we have 
\begin{align*} &r_{0} - O(1/n^{1/d_z}) \leq  \hat{R}  \leq r_{0} + \mathcal{O}(1/n^{1/d_z}) + \mathcal{O}\left(\sqrt{V} \left( n^{-1/3} + \sqrt{2^{d_z}/n} \right)\right) \end{align*}
with high probability, upto log factors. Here $r_0 = 0.5(1 - d_{TV}(f,f^{CI}))$, $V$ is the VC dimension~\cite{vapnik2015uniform} of the class $\mathcal{G}$.  Thus when $f$ is equivalent to $f^{CI}$ ($\mathcal{H}_0$ holds) then the error rate of the classifier is close to $0.5$. But when $\mathcal{H}_1$ holds the loss is much lower.  We provide a novel analysis of Rademacher complexity bounds~\cite{boucheron2005theory} under near-independence which is of independent interest. 

$(iv)$ {\bf (Empirical Evaluation)} We perform extensive numerical experiments where our algorithm outperforms the state of the art~\cite{zhang2012kernel,strobl2017approximate}. We also apply our algorithm for analyzing CI relations in the protein signaling network  data from the flow cytometry data-set~\cite{sachs2005causal}. In practice we observe that the performance with respect to dimension of $Z$ scales much better than expected from our worst case theoretical analysis. This is because powerful binary classifiers perform well in high-dimensions. 





















%The main contributions of this paper are as follows:
%
%$(i)$ {\bf (Nearest-Neighbor Bootstrap)} We propose a nearest-neighbor based bootstrap method to produce samples whose distributions are close to $f^{CI}$, given access to $n$ i.i.d samples from the joint $f_{X,Y,Z}(x,y,z)$. This is Algorithm~\ref{alg:NNB} in our paper. We prove that the variational distance between the distribution of any one of the samples returned by Algorithm~\ref{alg:NNB} and $f^{CI}$ (conditionally independent distribution) is $O((1/n)^{1/2d_z})$ under mild smoothness assumptions on $f_{X,Y,Z}(x,y,z)$. 
%
%$(ii)$ {\bf (Reduction to Classification)} We reduce the problem of CI tests into a binary classification problem, through our nearest neighbor bootstrap. As shown in Fig.~\ref{fig:illustrate}, we withhold $n/3$ of the original samples in data-set $\mathcal{U}$, while $2n/3$ of the original samples are passed through the nearest neighbor boot-strap to create $n/3$ samples (in $\mathcal{U}'$), that are close to $f^{CI}$ in distribution.  The samples in $\mathcal{U}$ are labeled $1$ and the ones in $\mathcal{U}'$ are labeled $0$. This labeled data-set is broken into training set $\mathcal{D}_r$ and test set $\mathcal{D}_e$. A classifier $\hat{g}$ is trained on $\mathcal{D}_r$. 
%
%The key idea is that if the original samples are in fact CI ($\mathcal{H}_0$ holds), then the two data-sets cannot be distinguished and the test error $\hat{L}(\hat{g},\mathcal{D}_{e})$ will be close to $0.5$ (random guessing). However, if $\mathcal{H}_1$ holds, then the classifier will be able to differentiate between the data-sets i.e. $\hat{L}(\hat{g},\mathcal{D}_{e}) < 0.5$ would be observed. We provide a detailed pseudo-code in Algorithm~\ref{alg:ccitv1}.
%
%$(iii)$ {\bf (Bias Corrected Algorithm)} We provide an improved algorithm in Algorithm~\ref{alg:ccitv2}. The samples generated in the nearest-neighbor boot-strap are close to $f^{CI}$ but the variational distance is not exactly equal to $0$ for finite $n$. Moreover the bootstrapped samples are not exactly i.i.d. Therefore, the trained classifier is expected to have a bias i.e the classifier can achieve a test loss slightly less than 0.5, even when $\mathcal{H}_0$ holds. In Algorithm~\ref{alg:ccitv2}, we propose a simple idea to rectify this bias.  
%
%%(i) a part of the original i.i.d samples are labeled $1$ (ii) the other part of the original samples are supplied to Algorithm~\ref{alg:NNB} to produce samples that are close to $f^{CI}$. These new samples are labeled $0$. (iii) A subset labeled samples are supplied to a binary classifier for training. The trained classifier is tested on a validation set (separate from the training set). If the trained classifier has good accuracy over a validation set, then intuitively it means that the joint distribution $f_{X,Y,Z}(.)$ is distinguishable from $f^{CI}$ (note that the generated samples labeled 0 are close in distribution to $f^{CI}$). Therefore, we reject $\mathcal{H}_0$. On the other hand, if the classifier has accuracy close to random guessing, then $f_{X,Y,Z}(.)$ is in fact close to $f^{CI}$, and we fail to reject $\mathcal{H}_0$.
%
%$(iv)$ {\bf (Novel Generalization Guarantees for Classification)} The samples generated by the nearest-neighbor bootstrap are not i.i.d any more, but they are \textit{close} to i.i.d. We show that even though these samples are not i.i.d, generalization bounds (similar to~\cite{boucheron2005theory} ) for the risk of classifiers trained on them, still hold. (add details about the result). In proving this, we provide a novel analysis for Rademacher type bounds (refer to ~\cite{boucheron2005theory}) for non-i.i.d samples, which relate the classification accuracy to the number of samples and the $VC$-dimension~\cite{vapnik2015uniform} of the class of functions in the classifier. This analysis technique may be of independent interest. 
%
%$(v)$ {\bf (Empirical Validation)} We perform better on real and simulated data..........need more evidence to write. 
%


==> Introductionv6.tex <==
%Rough Story....
%
%(i) Three areas where CI tests are the main work-horse:
%
%(1) Markov Blanket Estimation with cites.
%
%(2) Bayesian Network Learning - add cites
%
%(3) Causal Structure learning - discuss both constraint based and score based contributions. 
%
%Prior work on parametric and non-parametric CI. Kernel based methods. Discuss run time and dimensionality hit. 
%
%(ii) Discuss that ours is a modular approach- simple bootstrap followed by powerful classifiers. Classifiers can be flexibly chosen with domain knowledge, and any advancement in this field implies an advancement in ours. Discuss dimension issues. 
%
%(iii) List main contributions:
%
%(1) Reduction to classification with NNB.
%
%(2) Guarantees for NNB
%
%(3) Novel guarantees for non-i.i.d classification
%
%(4) Empirical Performance. 

%%%%%%%%%%%%%%%%%%%%%%%%%Start Intro%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
Testing datasets for conditional independence have significant
applications in several statistical/learning applications; among
others, examples include discovering/testing for edges in Bayesian
networks~\cite{koller2009probabilistic,
  spirtes2000causation,cheng1998learning,de2000new}, causal
inference~\cite{pearl2009causality,
  kalisch2007estimating,tsamardinos2006max, brenner2013sparsityboost}
and feature selection through Markov
Blankets~\cite{koller1996toward,xing2001feature}. Given a set of
triplets of random variables/vectors $(X, Y, Z)$, we say that $X$ is
conditionally independent of $Y$ given $Z$ (denoted by
$X \independent Y \vert Z$), if the joint distribution
$f_{X,Y,Z}(x,y,z)$ factorizes as
$f_{X,Y,Z}(x,y,z) = f_{X|Z}(x|z)f_{Y|Z}(y|z)f_{Z}(z)$. The problem of
\textit{Conditional Independence Testing} (CI Testing) can be defined
as follows: Given $n$ i.i.d samples from $f_{X,Y,Z}(x,y,z)$,
distinguish between the two hypothesis $\mathcal{H}_0:$
$X \independent Y \vert Z$ and $\mathcal{H}_1:$
$X \centernot{\independent} Y \vert Z$.

% CI tests are fundamental tools for learning Bayesian
% networks~\cite{koller2009probabilistic}, causal
% inference~\cite{pearl2009causality} and feature selection through
% Markov Blankets~\cite{koller1996toward}. In causal structure learning,
% results of CI tests among the nodes of a causal
% graph~\cite{pearl2009causality} are vital inputs to popular constraint
% based algorithms~\cite{kalisch2007estimating,tsamardinos2006max}. A
% key property is that given two variables on a causal graph $X$ and $Y$
% and a vector of other variables $Z$ (vector of nodes in the causal
% graph), $X \independent Y \vert Z$, implies the absence of an edge
% between $X$ and $Y$. Some of the more recent score-based methods of
% causal inference also rely on effective CI
% tests~\cite{brenner2013sparsityboost}. Similarly in the field of
% learning Bayesian networks, results from CI tests are used to discover
% edges between random variables that form the nodes of the
% network~\cite{spirtes2000causation,cheng1998learning,de2000new}. CI
% tests are also useful in the field of feature selection for
% high-dimensional supervised learning problems through Markov
% blankets~\cite{koller1996toward, xing2001feature}. 


% It is important to note that in many of these settings, while $X,Y$
% might be low-dimensional, $Z$ is high-dimensional due to the size of
% the conditioning set that potentially separates $(X,Y)$ from the rest
% of the graph.

In this paper we propose a data-driven \textit{Model-Powered} CI test. The central idea in a model-driven approach is to convert a statistical testing or estimation problem into a pipeline that utilizes the power of supervised learning models like classifiers and regressors, that have attractive properties especially in high-dimensions. In this paper, we take such a model-powered approach (illustrated in
Fig.~\ref{fig:illustrate}), which reduces the problem of CI testing to
Binary Classification. Specifically, the key steps of our procedure are as follows:

%Our approach is inspired by Classifier Two-Sample
%tests~\cite{LopezPaz,OthersBBB} which use this approach for
%independence testing and two-sample tests. We start by understanding
%how to build a model-powered independence test. For two random
%variables $X,Y$ we are given i.i.d. samples $(X_i,Y_i)$,
%$i=1 \ldots n/2$ and we would like to know if $X$ is independent from
%$Y$. To achieve this, we split the samples in half: for the first half
%simply add the label $y=0$ for $i=1 \ldots n/2$, indicating unshuffled
%data. For the other half, we randomly permute $Y_i$, i.e. create
%$(X_i, Y_{\pi (i)})$, $i= n/2, \ldots n$, for a random permutation
%$\pi(i)$ and add the label $Y=1$, i.e. mark them as shuffled. Now we
%give half of the shuffled and half the unshuffled data to a classifier
%that tries to learn to predict if a tuple is shuffled, or not. We can
%subsequently use the remaining data to test the model accuracy. If the
%model can confidently distinguish between shuffled and un-shuffled
%$(X_i,Y_i)$ tuples, this proves that $X$ and $Y$ are not independent.
%Note that, as usual, we can never confidently show that $X$ and $Y$
%\textit{are} independent since our model may be weak and fail to
%capture some complex dependency structure between $X$ and $Y$. For
%this reason we can confidently reject (or fail to reject) the
%independence Null hypothesis and $p$-values can be easily obtained
%since the model would be performing random guesses under the Null.
%
%Conditional independence testing is fundamentally harder than
%independence testing (see e.g.~\cite{bergsma2004testing}). When $Z$ is
%discrete, CI tests can be reduced to multiple independence tests, one
%for each value of $Z$. The continuous setting is more challenging and
%previous methods often rely on parametric assumptions like linear
%relations between the random variables with additive Gaussian noise,
%where the problem reduces to testing for
%correlations~\cite{lawrance1976conditional}. Our focus is on
%\textit{non-parametric} CI testing for continuous random variables,
%i.e. determining CI relations under minimal simplifying assumptions.
%
%Some of the earlier methods for non-parametric CI testing, either
%involve discretizing $Z$ into sets of
%bins~\cite{margaritis2005distribution}, or involve estimating the
%marginal densities $f_{X \vert Z}(.)$ and
%$f_{Y \vert Z}(.)$~\cite{su2007consistent}. Unfortunately, these
%methods do not perform well in higher dimensions of $Z$. Recently,
%powerful kernel based methods for non-parametric CI testing have been
%proposed that are accurate even for moderate values of the dimensions
%of
%$Z$~\cite{gao2016demystifying,strobl2017approximate,zhang2012kernel,doran2014permutation}.
% Many of these approaches are based on the observation
% in~\cite{fukumizu2004dimensionality}, that non-parametric CI
% relations can be characterized using covariance operators in the
% reproducing kernel Hilbert spaces (RKHS).
%However, even these kernel based methods have issues in accuracy of
%the test when the dimension of the conditioning set is
%large~\cite{doran2014permutation} and also incur prohibitive running
%times when the number of samples ($n$) is
%large~\cite{strobl2017approximate}.

\begin{figure}[h] \centering
  \includegraphics[width=8cm,height=4.5cm]{illustrate.pdf}
  \caption{Illustration of our methodology. A part of the original
    samples are kept aside in $\mathcal{U}_1$. The rest of the samples
    are used in our nearest neighbor boot-strap to generate a data-set
    $\mathcal{U}_2'$ which is close to $f^{CI}$ in distribution. The
    samples are labeled as shown and a classifier is trained on a
    training set. The test error is measured on a test set
    there-after. If the test-error is close to $0.5$, then
    $\mathcal{H}_0$ is not rejected, however if the test error is low
    then $\mathcal{H}_0$ is rejected.}
	\label{fig:illustrate}
\end{figure}



%For vanilla independence testing, the key
%property was that the permuted tuples $(X_i,Y_{\pi(i)})$ are i.i.d.
%samples from the product distribution density $f(x)f(y)$. It is quite
%interesting that a permutation allows us create samples from
%$f(x)f(y)$ without needing to learn these potentially high-dimensional
%distributions. To perform conditional independence tests we have to
%solve the analogous problem: we need to create samples from the
%conditional product distribution $f^{CI}(x,y,z) = f(x|z)f(y|z)f(z)$,
%given access only to i.i.d. samples from the joint distribution
%$f(x,y,z)$. Our key technical contribution is to show how this can be
%done with a nearest-neighbor bootstrap procedure and establish that
%these are close in total variation distance to the true $f^{CI}$
%distribution.
 
\setword{$(i)$}{step1}
Suppose we are provided $3n$ i.i.d
samples from $f_{X,Y,Z}(x,y,z)$. We keep aside $n$ of these original samples in a set $\mathcal{U}_1$ (refer to Fig.~\ref{fig:illustrate}).
The remaining $2n$ of the original samples are processed through our
first module, the \textit{nearest-neighbor bootstrap} (Algorithm~\ref{alg:NNB} in our paper), which produces $n$
simulated samples stored in $\mathcal{U}_2'$. In
Section~\ref{sec:results}, we show that the generated samples in
$\mathcal{U}_2'$ are in fact close in total variational distance
(defined in Section~\ref{sec:results}) to the distribution
$f^{CI}(x,y,z) \triangleq f_{X|Z}(x|z)f_{Y|Z}(y|z)f_Z(z)$. Note that
$f^{CI}(.) = f_{X,Y,Z}(.)$ when $\mathcal{H}_0$ holds.


\setword{$(ii)$}{step2} Subsequently, the original samples kept aside
in $\mathcal{U}_1$ are labeled $1$ while the new samples simulated
from the nearest-neighbor bootstrap (in $\mathcal{U}_2'$) are labeled
$0$. The labeled samples ($\mathcal{U}_1$ with label $1$ and
$\mathcal{U}_2'$ labeled 0) are aggregated into a data-set
$\mathcal{D}$. $\mathcal{D}$ is then broken into training and test
sets $\mathcal{D}_r$ and $\mathcal{D}_e$ each containing $n$ samples
each.

\setword{$(iii)$}{step3} Given the labeled training data-set (from
step~\ref{step2}), we train powerful classifiers such as gradient boosted
trees~\cite{chen2016xgboost} or deep neural
networks~\cite{krizhevsky2012imagenet} which attempt to learn the
classes of the samples. If the trained classifier has good accuracy
over the test set, then intuitively it means that the joint
distribution $f_{X,Y,Z}(.)$ is distinguishable from $f^{CI}$ (note
that the generated samples labeled 0 are close in distribution to
$f^{CI}$). Therefore, we reject $\mathcal{H}_0$. On the other hand, if
the classifier has accuracy close to random guessing, then
$f_{X,Y,Z}(.)$ is in fact close to $f^{CI}$, and we fail to reject
$\mathcal{H}_0$.

For independence testing (i.e whether $X \independent Y$), classifiers were recently used in~\cite{lopez2016revisiting}. Their key observation was that given i.i.d samples $(X,Y)$ from $f(x,y)$, if the $Y$ coordinates are randomly permuted then the resulting samples exactly emulate the distribution $f_X(x)f_Y(y)$. Thus the problem can be converted to a two sample test between a subset of the original samples and the other subset which is permuted - Binary classifiers were harnessed for this two-sample testing. However, in the case of CI testing we need to emulate samples from $f^{CI}$. This is much harder inherently as now the permutation of the samples needs to be $Z$ dependent (which can be high-dimensional). One of our key technical contribution is proving that our nearest-neighbor bootstrap in step~\ref{step1} achieves this task. 

The advantage of this modular approach is that we can harness the power of classifiers (in step~\ref{step3} above), which have good accuracies in high-dimensions. Thus, any improvements in the field of binary classification imply an advancement in our CI test. Moreover, there is added flexibility in choosing the best classifier based on domain knowledge about the data-generation process. Finally, our bootstrap is also efficient owing to fast algorithms for identifying nearest-neighbors~\cite{ramasubramanian1992fast}. 

\subsection{Main Contributions}
\label{contri}
$(i)$ {\bf (Classification based CI testing)} We reduce the problem of CI testing to Binary Classification as detailed in steps~\ref{step1}-\ref{step3} above and in Fig.~\ref{fig:illustrate}. We simulate samples that are close to $f^{CI}$ through a novel nearest-neighbor bootstrap (Algorithm~\ref{alg:NNB}) given access to i.i.d samples from the joint distribution. The problem of CI testing then reduces to a two-sample test between the original samples in $\mathcal{U}_1$ and $\mathcal{U}_2'$, which can be effectively done by binary classifiers.

$(ii)$ {\bf (Guarantees on Bootstrapped Samples)} As mentioned in steps~\ref{step1}-\ref{step3}, if the samples generated by the bootstrap (in $\mathcal{U}_2'$) are close to $f^{CI}$, then the CI testing problem reduces to testing whether the data-sets $\mathcal{U}_1$ and $\mathcal{U}_2'$ are distinguishable from each other.  We theoretically justify that this is indeed true. Let $\phi_{X,Y,Z}(x,y,z)$ denote the distribution of a sample produced by Algorithm~\ref{alg:NNB}, when it is supplied with $n$ i.i.d  samples from $f(x,y,z)$. In Theorem~\ref{thm:dtv}, we prove that $d_{TV}(\phi, f^{CI}) = O(1/n^{1/d_z})$ under appropriate smoothness assumptions. Here $d_z$ is the dimension of $Z$ and $d_{TV}$ denotes total variational distance (Def.~\ref{dtv}). 

%One of our main theoretical results is that the marginal distribution of a sample generated by the nearest-neighbor bootstrap is close in variational distance to the conditionally independent distribution $f^{CI}$. Let $\phi_{X,Y,Z}(x,y,z)$ denote the distribution of a sample produced by Algorithm~\ref{alg:NNB}, when it is supplied with $n$ i.i.d  samples from $f(x,y,z)$. In Theorem~\ref{thm:dtv}, we prove that $d_{TV}(\phi, f^{CI}) = O(1/n^{1/d_z})$ under appropriate smoothness assumptions. Here $d_z$ is the dimension of $Z$ and $d_{TV}$ denotes total variational distance (Def.~\ref{dtv}).

$(iii)$ {\bf (Generalization Bounds for Classification under \textit{near-independence})} The samples generated from the nearest-neighbor bootstrap do not remain i.i.d but they are \textit{close} to i.i.d. We quantify this property and go on to show generalization risk bounds for the classifier. Let us denote the class of function encoded by the classifier as $\mathcal{G}$. Let $\hat{R}$ denote the probability of error of the optimal classifier $\hat{g} \in \mathcal{G}$ trained on the training set (Fig.~\ref{fig:illustrate}). We prove that under appropriate assumptions, we have 
\begin{align*} &r_{0} - O(1/n^{1/d_z}) \leq  \hat{R}  \leq r_{0} + \mathcal{O}(1/n^{1/d_z}) + \mathcal{O}\left(\sqrt{V} \left( n^{-1/3} + \sqrt{2^{d_z}/n} \right)\right) \end{align*}
with high probability, upto log factors. Here $r_0 = 0.5(1 - d_{TV}(f,f^{CI}))$, $V$ is the VC dimension~\cite{vapnik2015uniform} of the class $\mathcal{G}$.  Thus when $f$ is equivalent to $f^{CI}$ ($\mathcal{H}_0$ holds) then the error rate of the classifier is close to $0.5$. But when $\mathcal{H}_1$ holds the loss is much lower.  We provide a novel analysis of Rademacher complexity bounds~\cite{boucheron2005theory} under near-independence which is of independent interest. 

$(iv)$ {\bf (Empirical Evaluation)} We perform extensive numerical experiments where our algorithm outperforms the state of the art~\cite{zhang2012kernel,strobl2017approximate}. We also apply our algorithm for analyzing CI relations in the protein signaling network  data from the flow cytometry data-set~\cite{sachs2005causal}. In practice we observe that the performance with respect to dimension of $Z$ scales much better than expected from our worst case theoretical analysis. This is because powerful binary classifiers perform well in high-dimensions. 





















%The main contributions of this paper are as follows:
%
%$(i)$ {\bf (Nearest-Neighbor Bootstrap)} We propose a nearest-neighbor based bootstrap method to produce samples whose distributions are close to $f^{CI}$, given access to $n$ i.i.d samples from the joint $f_{X,Y,Z}(x,y,z)$. This is Algorithm~\ref{alg:NNB} in our paper. We prove that the variational distance between the distribution of any one of the samples returned by Algorithm~\ref{alg:NNB} and $f^{CI}$ (conditionally independent distribution) is $O((1/n)^{1/2d_z})$ under mild smoothness assumptions on $f_{X,Y,Z}(x,y,z)$. 
%
%$(ii)$ {\bf (Reduction to Classification)} We reduce the problem of CI tests into a binary classification problem, through our nearest neighbor bootstrap. As shown in Fig.~\ref{fig:illustrate}, we withhold $n/3$ of the original samples in data-set $\mathcal{U}$, while $2n/3$ of the original samples are passed through the nearest neighbor boot-strap to create $n/3$ samples (in $\mathcal{U}'$), that are close to $f^{CI}$ in distribution.  The samples in $\mathcal{U}$ are labeled $1$ and the ones in $\mathcal{U}'$ are labeled $0$. This labeled data-set is broken into training set $\mathcal{D}_r$ and test set $\mathcal{D}_e$. A classifier $\hat{g}$ is trained on $\mathcal{D}_r$. 
%
%The key idea is that if the original samples are in fact CI ($\mathcal{H}_0$ holds), then the two data-sets cannot be distinguished and the test error $\hat{L}(\hat{g},\mathcal{D}_{e})$ will be close to $0.5$ (random guessing). However, if $\mathcal{H}_1$ holds, then the classifier will be able to differentiate between the data-sets i.e. $\hat{L}(\hat{g},\mathcal{D}_{e}) < 0.5$ would be observed. We provide a detailed pseudo-code in Algorithm~\ref{alg:ccitv1}.
%
%$(iii)$ {\bf (Bias Corrected Algorithm)} We provide an improved algorithm in Algorithm~\ref{alg:ccitv2}. The samples generated in the nearest-neighbor boot-strap are close to $f^{CI}$ but the variational distance is not exactly equal to $0$ for finite $n$. Moreover the bootstrapped samples are not exactly i.i.d. Therefore, the trained classifier is expected to have a bias i.e the classifier can achieve a test loss slightly less than 0.5, even when $\mathcal{H}_0$ holds. In Algorithm~\ref{alg:ccitv2}, we propose a simple idea to rectify this bias.  
%
%%(i) a part of the original i.i.d samples are labeled $1$ (ii) the other part of the original samples are supplied to Algorithm~\ref{alg:NNB} to produce samples that are close to $f^{CI}$. These new samples are labeled $0$. (iii) A subset labeled samples are supplied to a binary classifier for training. The trained classifier is tested on a validation set (separate from the training set). If the trained classifier has good accuracy over a validation set, then intuitively it means that the joint distribution $f_{X,Y,Z}(.)$ is distinguishable from $f^{CI}$ (note that the generated samples labeled 0 are close in distribution to $f^{CI}$). Therefore, we reject $\mathcal{H}_0$. On the other hand, if the classifier has accuracy close to random guessing, then $f_{X,Y,Z}(.)$ is in fact close to $f^{CI}$, and we fail to reject $\mathcal{H}_0$.
%
%$(iv)$ {\bf (Novel Generalization Guarantees for Classification)} The samples generated by the nearest-neighbor bootstrap are not i.i.d any more, but they are \textit{close} to i.i.d. We show that even though these samples are not i.i.d, generalization bounds (similar to~\cite{boucheron2005theory} ) for the risk of classifiers trained on them, still hold. (add details about the result). In proving this, we provide a novel analysis for Rademacher type bounds (refer to ~\cite{boucheron2005theory}) for non-i.i.d samples, which relate the classification accuracy to the number of samples and the $VC$-dimension~\cite{vapnik2015uniform} of the class of functions in the classifier. This analysis technique may be of independent interest. 
%
%$(v)$ {\bf (Empirical Validation)} We perform better on real and simulated data..........need more evidence to write. 
%


==> Psetting.tex <==

{\bf Problem Setting: }The problem setting is that of non-parametric \textit{Conditional Independence (CI)} testing given i.i.d samples from the joint distributions of random variables/vectors~\cite{zhang2012kernel,doran2014permutation,strobl2017approximate}. We are given $n$ i.i.d samples from a continuous joint distribution $f_{X,Y,Z}(x,y,z)$ where $x \in \mathbb{R}^{d_x}, y \in \mathbb{R}^{d_y}$ and $z \in \mathbb{R}^{d_z}$. The goal is to test whether $X \independent Y \vert Z$ i.e whether $f_{X,Y,Z}(x,y,z)$ factorizes as,
$f_{X,Y,Z}(x,y,z) = f_{X \vert Z}(x \vert z)f_{Y \vert Z}(y \vert z)f_{Z}(z) \label{eq:CI} \triangleq f^{CI}(x,y,z)$

This is essentially a hypothesis testing problem where: $\mathcal{H}_0 \text{ : } X \independent Y \vert Z$ and 
$\mathcal{H}_1 \text{ : } X \centernot{\independent} Y \vert Z$.

%Prior methods for this binary hypothesis testing problem involve kernel based techniques that estimate the marginal distributions of $X$ and $Y$ given $Z$~\cite{zhang2012kernel,doran2014permutation,strobl2017approximate,gao2016demystifying}. In this paper our goal is to convert this problem into a binary classification setting, which enables us to use powerful supervised learning models like gradient-boosted trees or deep neural networks. 

{\bf Note: } For notational convenience, we will drop the subscripts when the context is evident. For instance we may use $f(x \vert z)$ in place of $f_{X \vert Z}(x \vert z)$. 

%\subsection{Reduction to Classification}
%\label{sec:red_class}
%{\color{red} This is repeated too much. Need to integrate this in the contributions or the introduction.} 
%
%In this paper we convert the binary hypothesis testing problem of CI tests into a classification scenario. Similar ideas have been used in~\cite{lopez2016revisiting} in the context of testing whether two jointly distributed random variables/vectors $X$ and $Y$ are independent. 
%
%Let $\mathcal{U} := \{u_i := (x_i,y_i,z_i) \}_{i=1}^{n}$ denote the data-set consisting of $n$ i.i.d samples that were originally supplied. The goal is to use these samples in order to create another data-set which mimics i.i.d samples generated from the distribution $f^{CI}(x,y,z) := f_{X \vert Z}(x \vert z)f_{Y \vert Z}(y \vert z)f_{Z}(z)$. Let this generated data-set be denoted by $\mathcal{U'} := \{u'_i := (x'_i,y'_i,z'_i) \}_{i=1}^{n'}$, where $n' < n$. Using these two data-sets we create a labeled data-set as follows:
%\begin{align}
%\mathcal{D} := \{ (u_i,\ell_i = 1)\}_{\{u_i \in \mathcal{U}: i \in \{1,\cdots,n' \}\}} \cup \{ (u',\ell' = 0)\}_{u' \in \mathcal{U'}}
%\end{align}
%such that the original samples are labeled as $1$ while the generated samples mimicking the distribution $f^{CI}$ are labeled $0$. The labeled data-set $\mathcal{D}$ is randomly partitioned into two data-sets $D_{r}$ and $D_{e}$ for training and testing respectively. Now, a binary classifier $g:\mathbb{R}^{d_x+d_y+d_z} \rightarrow \{0,1\}$ is trained using $D_{r}$ and the test misclassification rate $\hat{L}(g,\mathcal{D}_{e}) = \sum _{(u,l) \in \mathcal{D}_{e}}\mathds{1} \{g(u) \neq l \}$ is calculated using $D_{e}$. 
%
%The key idea is that if the original samples are in fact CI ($\mathcal{H}_0$ holds), then the two data-sets cannot be distinguished and $\hat{L}(g,\mathcal{D}_{e})$ will be that of random guessing that is $0.5$. On the other hand if $\mathcal{H}_1$ is true, then the classifier will be able to differentiate between the data-sets and $\hat{L}(g,\mathcal{D}_{e}) < 0.5$ would be observed. The main challenge is to simulate $\mathcal{U}'$ using i.i.d samples from the joint. We describe a nearest-neighbor bootstrap approach for the same and also formalize the CI testing algorithm in the next section. 

==> Results.tex <==
In this section, we provide our main theoretical results. We first show that the distribution of any one of the samples generated in Algorithm~\ref{alg:NNB} closely resemble that of a sample coming from $f^{CI}$. This result holds for a broad class of distributions $f_{X,Y,Z}(x,y,z)$ which satisfy some smoothness assumptions. However, the samples generated by Algorithm~\ref{alg:NNB} ($\mathcal{U}_2$ in the algorithm) are not exactly i.i.d but \textit{close} to i.i.d. We quantify this and go on to show that empirical risk minimization over a class of classifier functions generalizes well using these samples. We provide a novel analysis which provides Rademacher complexity type bounds~\cite{boucheron2005theory} for these non i.i.d samples. %Finally, we theoretically justify our bias correction in Algorithm~\ref{alg:ccitv2}. 
Before, we formally state our results we provide some useful definitions. 

\begin{definition} (Total Variational Distance) \label{dtv} The total variational distance between two continuous probability distributions $f(.)$ and $g(.)$ defined over a domain $\mathcal{X}$ is given by,
	\begin{equation}
	d_{TV}(f,g) = \frac{1}{2} \int_{x \in \mathcal{X}} \lvert f(x) - g(x) \rvert dx
	\end{equation}
\end{definition}

%\begin{definition} (Kullback–Leibler divergence) The KL-divergence between two continuous probability distributions $f(.)$ and $g(.)$ defined over a domain $\mathcal{X}$ is given by,
%	\begin{equation}
%	\mathrm{KL}(f \Vert g) = \int_{x \in \mathcal{X}} f(x) \log \left( \frac{f(x)}{g(x)}\right) dx
%	\end{equation}
%\end{definition}

%\begin{definition}
%	(Fisher Information Matrix) Let $\mathbf{I}(z)$ be the Fisher information matrix of the parameterized distributions $f(y|z)$. The fisher information defines the curvature of the relative entropy, such that:
%	\begin{equation}
%	 \mathbf{I}(z)_{ij} = \EE \left[ -\frac{\delta^2 \log f(y|z)}{\delta z_i \delta z_j} \Bigg \vert Z = z\right] = \left(\frac{\partial^2}{\partial z'_i \partial z'_j} \int \log \frac{f(y|z)}{f(y|z')}  f(y|z) dy \right) \Bigg \vert _{z' = z}
%	\end{equation}
%\end{definition}

Now we are at a position to state one of our main results. We prove that the distribution of any one of the samples generated in Algorithm~\ref{alg:NNB} is close to $f^{CI}$ in terms of total variational distance. We make the following assumptions on the joint distribution of the original samples i.e. $f_{X,Y,Z}(x,y,z)$:

{\bf Smoothness assumption on $f(y|z)$: } We assume the following smoothness condition on $f(y|z)$. This is slight generalization of requiring the maximum eigenvalue of Fisher Information matrix of $y$ with respect to $z$ to be bounded.
\begin{assumption}
	\label{assump1}
	For $z \in \mathbb{R}^{d_z}$  and $a$ such that $\lVert a - z \rVert_2 \leq \epsilon_1$, let us define the generalized curvature matrix $\mathbf{I}_{a}(z)$ as,
	\begin{equation}
	\mathbf{I}_{a}(z)_{ij} = \left(\frac{\partial^2}{\partial z'_i \partial z'_j} \int \log \frac{f(y|z)}{f(y|z')}  f(y|z) dy \right) \Bigg \vert _{z' = a} = \EE \left[ -\frac{\delta^2 \log f(y|z')}{\delta z'_i \delta z'_j} \Big \vert _{z' = a} \Bigg \vert Z = z\right]
	\end{equation}
	We require that for all $z \in \mathbb{R}^{d_z}$ and all $a$ such that $\lVert a - z \rVert_2 \leq \epsilon_1$, $\lambda_{max} \left( \mathbf{I}_{a}(z) \right) \leq \beta$.
\end{assumption}

{\bf Smoothness assumptions on $f(z)$: }
We assume some smoothness properties of the probability density function $f(z)$. The smoothness assumptions (in Assumption~\ref{assumption1}) is a subset of the assumptions made in \cite{gao2016demystifying} (Assumption 1, Page 5) for entropy estimation.

\begin{definition}
	For any $\delta >0$, we define  $G(\delta) = \PP \left( f(Z) \leq \delta \right)$. This is the probability mass of the distribution of $Z$ in the areas where the p.d.f is less than $\delta$. 
\end{definition}

\begin{definition}
(Hessian Matrix) Let $H_f(z)$ denote the Hessian Matrix of the p.d.f $f(z)$ with respect to $z$ i.e $H_f(z)_{ij} = \partial^2f(z)/\partial z_i \partial z_j$, provided it is twice continuously differentiable at $z$. 
\end{definition}

\begin{assumption}\label{assumption1}
	The probability density function $f(z)$ satisfies the following:
	
	(1) $f(z)$ is twice continuously differentiable and the Hessian matrix $H_f$ satisfies $\lVert H_f(z) \rVert_2 \leq c_{d_z}$ almost everywhere, where $c_{d_z}$ is only dependent on the dimension. 
	
	(2) $\int f(z)^{1-1/d} dz \leq c_3 ,~ \forall d \geq 2 $ where $c_3$ is a constant. 
\end{assumption}

\begin{theorem}
	\label{thm:dtv}
	Let $(X,Y',Z)$ denote a sample in $\mathcal{U}_2$ produced by Algorithm~\ref{alg:NNB} by modifying the original sample $(X,Y,Z)$ in $\mathcal{U}_1$, when supplied with $n$ i.i.d samples from the original joint distribution $f_{X,Y,Z}(x,y,z)$. Let $\phi_{X,Y,Z}(x,y,z)$ be the distribution of $(X,Y',Z)$. Under smoothness assumptions (\ref{assump1}) and (\ref{assumption1}), for any $\epsilon < \epsilon_1$, $n$ large enough, we have:
	\begin{align*}
	&d_{TV}(\phi,f^{CI}) \leq  b(n) \\
	&\triangleq  \frac{1}{2}\sqrt{\frac{\beta}{4} \frac{c_3 * 4^{1/d_z} \Gamma(1/d_z) }{(n \gamma_{d_z})^{1/d_z} d_z}  + \frac{\beta \epsilon G  \left(2c_{d_z} \epsilon^2 \right) }{4} }+  \exp \left( -\frac{1}{2}n \gamma_{d_z} c_{d_z} \epsilon^{d_z+2} \right) + G \left( 2 c_{d_z} \epsilon^2 \right).
	\end{align*}
	Here, $\gamma_d$ is the volume of the unit radius $\ell_2$ ball in $\mathbb{R}^d$.
\end{theorem}

Theorem~\ref{thm:dtv} characterizes the variational distance of the distribution of a sample generated in Algorithm~\ref{alg:NNB} with that of the conditionally independent distribution $f^{CI}$. Now, our goal is to characterize the test mis-classification error of the trained classifier in Algorithm~\ref{alg:ccitv1} under both $\mathcal{H}_0$ and $\mathcal{H}_1$. Consider the distribution of the samples in the data-set $\mathcal{D}_r$ used for classification in Algorithm~\ref{alg:ccitv1}. Let $q(x,y,z \vert \ell = 1)$ be marginal distribution of each sample with label $1$. Similarly, let $q(x,y,z \vert \ell = 0)$ denote the marginal distribution of the label $0$ samples. Note that under our construction, 
\begin{align*}
q(x,y,z \vert \ell = 1) &= f_{X,Y,Z}(x,y,z) = \left\{
\begin{array}{ll}
f^{CI}(x,y,z)  & \mbox{if } \mathcal{H}_0 \mbox{ holds }\\
\neq  f^{CI}(x,y,z) & \mbox{if }  \mathcal{H}_1 \mbox{ holds }
\end{array}
\right. \\
q(x,y,z \vert \ell = 0) &= \phi_{X,Y,Z}(x,y,z)   \numberthis \label{eq:classification}
\end{align*} 
where $\phi_{X,Y,Z}(x,y,z)$ is as defined in Theorem~\ref{thm:dtv}. 

Note that even though the marginal of each sample with label $0$ is $\phi_{X,Y,Z}(x,y,z)$ (Equation~\eqref{eq:classification}), they are not exactly i.i.d owing to the nearest neighbor bootstrap. We will go on to show that they are actually \textit{close} to i.i.d and therefore classification risk minimization generalizes similar to the i.i.d results for classification~\cite{boucheron2005theory}. However, before we go into our results we will include some insights from classification theory. 

{\bf Ideal Classification Setting:} We will consider an \textit{ideal} classification scenario for CI testing and in the process define standard quantities in learning theory. Recall that $\cG$ is the set of classifiers under consideration. Let $\tilde{q}$
be our \emph{ideal} distribution for $q$ given by $\tilde{q}(x,y,z|\ell=1) = f_{X,Y,Z}(x,y,z)$, $\tilde{q}(x,y,z|\ell=0) = f^{CI}_{X,Y,Z}(x,y,z)$ and $\tilde{q}(\ell=1) = \tilde{q}(\ell=0) = 0.5$. In other words this is the ideal classification scenario for testing CI. 
Let $L(g(\xyz),\ell) \triangleq \mathds{1}_{g(\xyz)\neq \ell}$ be our \textit{loss function} for a classifying function $g \in \mathcal{G}$, for a sample $u \triangleq (x,y,z)$.  For a distribution $\tilde{q}$ and a classifier $g$ let $R_{\tilde{q}}(g) \triangleq \EE_{u,\ell \sim \tilde{q}} [L(g(\xyz),\ell)]$ be the \textit{expected risk} of the function $g$. 
The \textit{risk optimal} classifier $g^*_{\tilde{q}}$ under $\tilde{q}$ is given by $g^*_{\tilde{q}} \triangleq \arg \min_{g \in \cG} R_{\tilde{q}}(g)$. Similarly for a set of samples $S$ and a classifier $g$, let $R_S(g) \triangleq \frac{1}{|S|}\sum_{u,\ell \in S} L(g(\xyz),\ell)$ be the \textit{empirical risk} on the set of samples. 
We define $g_S$ as the classifier that \textit{minimizes the empirical loss} on the observed set of samples $S$ that is,  $g_S \triangleq \arg \min_{g \in \cG} R_{S}(g)$.

If the samples in $S$ are generated independently from $\tilde{q}$, then
standard results from the learning theory states that with probability
$\geq 1-\delta$,
\[
R_{\tilde{q}}(g_S) \leq R_{\tilde{q}}(g^*_{\tilde{q}}) + C
\sqrt{\frac{V}{n}} + \sqrt{\frac{2 \log (1/\delta)}{n}}, \numberthis \label{eq:stdcc}
\]
where $V$ is the VC dimension~\cite{vapnik2015uniform} of the classification model, $C$ is
an universal constant and $n = \vert S \vert$. 

{\bf Non-i.i.d Samples:} In conditional independence testing, we do not have access
to samples from $\tilde{q}$. We sample from distribution $q$
given by Equation~\eqref{eq:classification}. In Theorem~\ref{thm:general} (in the appendix), we show that if samples in the training set $\mathcal{D}_r$ are
generated according to Algorithm~\ref{alg:NNB}, then 
\[
R_{q}(g_S) \leq R_{q}(g^*_q) + \gamma_n.  \numberthis \label{eq:main}
\]
under the conditions stated in Theorem~\ref{thm:short}. Since the loss function $L(.)$ is bounded by $1$, by Theorem~\ref{thm:dtv}, for any classifier $g$ $|R_{q}(g) - R_{\tilde{q}}(g)| \leq b(2n)$. Further, we have $|R_q(g^*_q) - R_{\tilde{q}}(g^*_{\tilde{q}})| \leq b(n)$ (proved in Lemma~\ref{lem:mindist}). Hence we have the following theorem, 
\begin{theorem}
	\label{thm:short}
	If the set of samples $S$ is generated from $q$ and $g_S$ satisfies conditions Theorem~\ref{thm:general}, then
	\[
	R_{\tilde{q}}(g_S) \leq R_{\tilde{q}}(g^*_{\tilde{q}}) + \gamma_n + 2 b(n)|L|.
	\]
\end{theorem}
Hence, our goal is Theorem~\ref{thm:general}. Note that unlike
standard tools from learning theory, the samples are not
independent. However, consider two sample inputs $u_i$ and $u_j$, such
that corresponding $z_i$ and $z_j$ are far away, then we expect the
resulting samples $u'_i$ and $u'_j$ to be nearly-independent. By
carefully, capturing this notion of spatial near-independence, we
prove generalization errors in Theorem~\ref{thm:general}. We note that
the notion of near-independence in terms of time has been used
in~\cite{mohri2009rademacher}


%\begin{definition}
%	(Bayes Optimal Classifier) Consider a binary classification problem consisting of samples and labels $\{x_i,\ell_i\}_{i=1}^{n}$ where $x_i \in \mathcal{X}$ and $\ell_i \in \{0,1\}$ for all $i$. Let $q(x \vert \ell = 1)$ and $q(x \vert \ell = 0)$ denote the distribution of the samples under the respective labels. Further, define $\eta(x) = \PP (\ell = 1 \vert X = x)$ i.e the probability of the label being $1$ given that the sample is $x$. Then, the Bayes Optimal classifier is defined as,
%	\begin{align*}
%	g^*(x) = \left\{
%	\begin{array}{ll}
%	1  & \mbox{if } \eta(x) \geq 0.5\\
%	0 & \mbox{if }  \eta(x) < 0.5   \numberthis
%	\end{array}
%	\right. \\
%	\end{align*}
%\end{definition}
%
%{\bf Fact:} For the above classification problem if $\PP(\ell = 0) = \PP(\ell = 1) = 0.5$, then the risk of Bayes Optimal classifier ($\PP(g^*(X) \neq \ell)$) is as follows:
%\begin{equation}
%\label{eq:bayes}
%\PP(g^*(X) \neq \ell) = \frac{1}{2} - \frac{1}{2} d_{TV}(q(x \vert \ell = 1),q(x \vert \ell = 0))
%\end{equation}
%where we use $\ell$ do also denote the random variable associated with the labels. No other classifier can have risk less than $g^*(.)$. 
%
%Now, we provide generalization bounds on the classification problem in Algorithm~\ref{alg:ccitv1}. We prove that under certain assumptions no classifier can have a good test mis-classification rate under $\mathcal{H}_0$. On the other hand, the empirical risk optimal classifier trained in Algorithm~\ref{alg:ccitv1} will have accuracy significantly less than $0.5$ under $\mathcal{H}_1$, provided some assumptions hold. Note, that the samples in $\mathcal{U}_2'$ are not i.i.d and therefore standard analysis for classification does not hold. We provide a novel analysis of Rademacher type bounds under non-i.i.d settings. 
%
%Before, we state our results, we briefly state the standard risk bounds for classification assuming i.i.d samples. Recall that $\cG$ is the set of classifiers under consideration. Let $\tilde{q}$
%be our \emph{ideal} distribution for $q$ given by
%\[
%\tilde{q}(x,y,z|\ell=1) = f_{X,Y,Z}(x,y,z),
%\]
%\[
%\tilde{q}(x,y,z|\ell=1) = f^{CI}_{X,Y,Z}(x,y,z),
%\]
%and $\tilde{q}(\ell=1) = \tilde{q}(\ell=0) = 0.5$. 
%Let $L(g(\xyz),\ell) = \mathds{1}_{g(\xyz)\neq \ell}$ be our loss function, where $u \triangleq (x,y,z)$.  For a distribution $q$ and a classifier $g$,
%let 
%\[
%R_{q}(g) = \EE_{u,\ell \sim \tilde{q}} [L(g(\xyz),\ell)].
%\]
%Let $g^*_{\tilde{q}}$ be the optimal
%classifier under $\tilde{q}$.
%\[
%g^*_{\tilde{q}} \triangleq \arg \min_{g \in \cG} R_{\tilde{q}}(g).
%\]
%Similarly for a set of samples $S$ and a claissifier $g$, let
%\[
%R_S(g) \triangleq \frac{1}{|S|}\sum_{u,\ell \in S} L(g(\xyz),\ell).
%\]
%Let $g_S$ be the classifier that minimizes the empirical loss on the
%observed set of samples, $S$ i.e.,
%\[
%g_S \triangleq \arg \min_{g \in \cG} R_{S}(g).
%\]
%If the set of samples $S$ are generated indepedently from $\tilde{q}$, then
%standard results from the learning theory states that with probability
%$\geq 1-\delta$,
%\[
%R_{\tilde{q}}(g_S) \leq R_{\tilde{q}}(g^*_{\tilde{q}}) + C
%\sqrt{\frac{V}{n}} + \sqrt{\frac{2 \log (1/\delta)}{n}},
%\]
%where $V$ is the VC dimension of the classification model and $C$ is
%some universal constant.
%
%However, in conditional independence testing, we do not have access
%for samples from $\tilde{q}$. Hence we sample from distribution $q$
%given by Equation~\eqref{eq:classification}.
%
%In Theorem~\ref{thm:general}, we show that if samples $S$ are
%generated according to Theorem~\ref{}, then 
%\[
%R_{q}(g_S) \leq R_{q}(g^*_q) + \gamma_n,
%\]
%Since the loss function $L$ is bounded, by Theorem~\ref{}, for any classifier $g$,
%\[
%|R_{q}(g) - R_{\tilde{q}}(g)| \leq b(n) |L|,
%\]
%where $|L|$ is the upper bound on $L$. Furthermore,
%\[
%|R_q(g^*_q) - R_{\tilde{q}}(g^*_{\tilde{q}})| \leq b(n) |L|.
%\]
%Hence, 
%\begin{theorem}
%	If $g_S$ satisfies Theorem~\ref{thm:general}, then
%	\[
%	R_{\tilde{q}}(g_S) \leq R_{\tilde{q}}(g^*_{\tilde{q}}) + \gamma_n + 2 b(n)|L|.
%	\]
%\end{theorem}
%Hence, our goal is Theorem~\ref{thm:general}. Note that unlike
%standard tools from learning theory, the samples are not
%independent. However, consider two sample inputs $u_i$ and $u_j$, such
%that corresponding $z_i$ and $z_j$ are far away, then we expect the
%resulting samples $u'_i$ and $u'_j$ to be nearly-independent. By
%carefully, capturing this notion of temporal near-independence, we
%prove generalization errors in Theorem~\ref{thm:general}. We note that
%the notion of near-indepence in terms of time has been used
%in~\cite{Mohri}





%The following are the main assumptions required from our generalization bounds:
%
%\begin{assumption}
%	\label{assum3}
%	We assume the following properties about the classification problem (\ref{eq:classification}) and the class of classifying function $\mathcal{G}$ (in Algorithm~\ref{alg:ccitv1}):
%	
%	(1) The Bayes Optimal Classifier $g^*$ of (\ref{eq:classification}) lies in our class of classification functions i.e. $g^* \in \mathcal{G}$.
%	
%	(2) The VC-dimension (\cite{vapnik2015uniform}) of the class of functions $\mathcal{G}$ is $V$.  
%\end{assumption}
%
%\begin{theorem}
%	Under Assumptions~\ref{assump1}, \ref{assumption1} and \ref{assum3}, we have the following results on the test classification error on the classifier $\hat{g}$ in Algorithm~\ref{alg:ccitv1}:
%	
%	(1) Under hypothesis $\mathcal{H}_0$, $\hat{L}(\hat{g},\mathcal{D}_{e}) > 0.5 - blah1$ with probability $1 - \delta$. 
%	
%	(2) Under hypothesis $\mathcal{H}_1$, $\hat{L}(\hat{g},\mathcal{D}_{e}) < 0.5 - blah2$ with probability $1 - \delta$. 
%\end{theorem}

==> Rwork.tex <==
In this paper we address the problem of non-parametric CI testing when the underlying random variables are continuous. The literature on non-parametric CI testing is vast. We will review some of the recent work in this field that is most relevant to our paper. 

Most of the recent work in CI testing are kernel based~\cite{strobl2017approximate,zhang2012kernel,doran2014permutation}. Many of these works   are based on the observation in~\cite{fukumizu2004dimensionality}, that non-parametric CI relations can be characterized using covariance operators in the reproducing kernel Hilbert spaces (RKHS). KCIT~\cite{zhang2012kernel} uses the partial association of regression functions relating $X$, $Y$ , and $Z$. RCIT~\cite{strobl2017approximate} is an approximate version of KCIT that attempts to improve running times when the number of samples are large. 
KCIPT~\cite{doran2014permutation} is perhaps most relevant to our work. In~\cite{doran2014permutation}, a specific permutation of the samples is used to simulate data from $f^{CI}$. An expensive linear program needs to be solved in order to calculate the permutation. On the other hand, we use a simple nearest-neighbor bootstrap and further we provide theoretical guarantees about the closeness of the samples to $f^{CI}$ in terms of total variational distance. Finally the two-sample test in~\cite{doran2014permutation} is based on a kernel method~\cite{borgwardt2006integrating}, while we use binary classifiers for the same purpose. There has also been some work on entropy estimation~\cite{gao2016demystifying} using nearest neighbor techniques, that can be used for CI testing by estimating the conditional mutual information $\mathrm{I}(X;Y \vert Z)$. 

Binary classification has been recently used for two-sample testing, in particular for independence testing~\cite{lopez2016revisiting}. Our analysis of generalization guarantees of classification are aimed at recovering guarantees similar to~\cite{boucheron2005theory}, but in a non-i.i.d setting. In this regard, there has been some recent work in proving Rademacher complexity bounds for $\beta$-mixing stationary processes~\cite{mohri2009rademacher}. 


